Robust No-Regret Learning in Min-Max Stackelberg Games

The behavior of no-regret learning algorithms is well understood in two-player min-max (i.e, zero-sum) games. In this paper, we investigate the behavior of no-regret learning in min-max games with dependent strategy sets, where the strategy of the first player constrains the behavior of the second. Such games are best understood as sequential, i.e., min-max Stackelberg, games. We consider two settings, one in which only the first player chooses their actions using a no-regret algorithm while the second player best responds, and one in which both players use no-regret algorithms. For the former case, we show that no-regret dynamics converge to a Stackelberg equilibrium. For the latter case, we introduce a new type of regret, which we call Lagrangian regret, and show that if both players minimize their Lagrangian regrets, then play converges to a Stackelberg equilibrium. We then observe that online mirror descent (OMD) dynamics in these two settings correspond respectively to a known nested (i.e., sequential) gradient descent-ascent (GDA) algorithm and a new simultaneous GDA-like algorithm, thereby establishing convergence of these algorithms to Stackelberg equilibrium. Finally, we analyze the robustness of OMD dynamics to perturbations by investigating online min-max Stackelberg games. We prove that OMD dynamics are robust for a large class of online min-max games with independent strategy sets. In the dependent case, we demonstrate the robustness of OMD dynamics experimentally by simulating them in online Fisher markets, a canonical example of a min-max Stackelberg game with dependent strategy sets.

==> Robust No-Regret Learning in Min Max Stackelberg Games (AAMAS 2022)/abstract.tex <==
\begin{abstract}
    The behavior of no-regret learning algorithms is well understood in two-player min-max (i.e, zero-sum) games. In this paper, we investigate the behavior of no-regret learning in min-max games \emph{with dependent strategy sets}, where the strategy of the first player constrains the behavior of the second. Such games are best understood as sequential, i.e., min-max Stackelberg, games. We consider two settings, one in which only the first player chooses their actions using a no-regret algorithm while the second player best responds, and one in which both players use no-regret algorithms. For the former case, we show that no-regret dynamics converge to a Stackelberg equilibrium. For the latter case, we introduce a new type of regret, which we call Lagrangian regret, and show that if both players minimize their Lagrangian regrets, then play converges to a Stackelberg equilibrium. We then observe that online mirror descent (OMD) dynamics in these two settings correspond respectively to a known nested (i.e., sequential) gradient descent-ascent (GDA) algorithm and a new simultaneous GDA-like algorithm, thereby establishing convergence of these algorithms to Stackelberg equilibrium. Finally, we analyze the robustness of OMD dynamics to perturbations by investigating online min-max Stackelberg games. We prove that OMD dynamics are robust for a large class of online min-max games with independent strategy sets. In the dependent case, we demonstrate the robustness of OMD dynamics experimentally by simulating them in online Fisher markets, a canonical example of a min-max Stackelberg game with dependent strategy sets.
\end{abstract}

==> Robust No-Regret Learning in Min Max Stackelberg Games (AAMAS 2022)/ack.tex <==
\begin{acks}
We thank several anonymous reviewers for their feedback on an earlier draft of this paper.

This work was partially supported by NSF Grant CMMI-1761546.
\end{acks}


==> Robust No-Regret Learning in Min Max Stackelberg Games (AAMAS 2022)/bounded-unbounded.tex <==
\section{No-Regret Learning Dynamics}
%in Min-Max Stackelberg games
\label{sec:no-regret}

In Stackelberg games, the outer player chooses their strategy assuming the inner player will best respond.
When both players' choices are optimal, the outcome is a Stackelberg equilibrium. 

In this section, we study no-regret learning dynamics in repeated min-max Stackelberg games in two settings: an \mydef{asymmetric} one in which the outer player is a no-regret learner while the inner player best-responds, and a \mydef{symmetric} one in which both players are no-regret learners.
Our main results are: 1.~In the asymmetric setting, if the outer player employs an asymmetric-regret-minimizing algorithm, play converges to a Stackelberg equilibrium, and 2.~in the symmetric setting, if both players employ a no-Lagrangian-regret algorithm, play converges to a Stackelberg equilibrium.

% \amy{should this assumption be moved to the end of the previous section, perhaps?}

% All the theoretical results in this paper rely on the following assumption(s):
%
% \begin{assumption}
% \label{main-assum}
% 1. (\emph{Slater's condition} \cite{slater1959convex, slater2014convex})~ $\forall \outer \in \outerset, \exists \widehat{\inner} \in \innerset$ s.t.\ $g_{\numconstr}(\outer, \widehat{\inner}) > \zeros$, for all $\numconstr = 1, \ldots, \numconstrs$; 2.~$\obj, \constr[1], \ldots, \constr[\numconstrs]$ are continuous and convex-concave; and 3.~$\grad[\outer] f, \grad[\outer] \constr[1], \ldots, \grad[\outer] \constr[\numconstrs]$ are well-defined for all $(\outer, \inner) \in \outerset \times \innerset$ and continuous in $(\outer, \inner)$; 4.~$\outerset$ and $\innerset$ are convex\deni{I cannot see this assumption stated anywhere oddly but it should be here!!} \amy{is this assumption missing from the NeurIPS paper as well?}\deni{Yes, it is missing but in the NeurIPS paper we state the convexity assumption in the theorem because it can be loosened sometimes, but we forget to state it for some lemmas, we have to fix that!}
% \end{assumption}
%
% We note that these assumptions are in line with previous work geared towards solving min-max Stackelberg games 
% %with first-order methods
% \cite{goktas2021minmax}.
% Part 1 of \Cref{main-assum},
% Slater's condition, is a standard constraint qualification condition \cite{boyd2004convex}, which is needed to derive the optimality conditions for the inner player's maximization problem; without it the problem becomes analytically intractable.
% Part 2 of \Cref{main-assum} ensures that the value function of the outer player is continuous and convex (\cite{goktas2021minmax}, Proposition A1), so that the problem affords an efficient solution.
% Part 3 of \Cref{main-assum} can be replaced by a weaker, subgradient boundedness assumption; however, for simplicity, we assume this stronger condition.
% Finally, Part 4 of \Cref{main-assum} guarantees that projections are polynomial-time operations.


\subsection{Asymmetric Learning Setting}

%\amy{i considered leader/follower. but it would be A LOT to change!!! and since Deni prefers it as is, i think it is probably best left as it was. but it is here now for you to read and form your own opinion.}\deni{I cannot decide this one. On one hand I agree that leader follower feels better in the learning framework but it feels disconnected from the min-max literature. }\sadie{Personally I slightly prefer the inner/outer player since leader/follower is not that compatible with the symmetric setting, while inner/outer can consistently work for both. But I do agree that leader/follower is better in the asymmetric setting.}\deni{Ah! This is such a great point Sadie!!! Let's stick to outer and inner!!}

We first consider an asymmetric setting in which the inner player best responds to the strategy picked by the outer player, while the outer player employs a no-regret learning algorithm. 
%%% pessimistic
In min-max Stackelberg games, the two players are adversaries, so this best-response assumption corresponds to the worst case.
In many real-world applications,  we seek optimal strategies for the outer player, e.g., in security games we are interested in an optimal strategy for the defender/outer player, not the attacker/inner player~\cite{kar2017trends}.
Assuming a strong inner player allows us to learn more robust 
%\amy{robust? i feel like it's more of a worst-case assumption than a robustness one.} \deni{Worst-case assumption is a robustness assumption for me, e.g., wald's min-max framework which is our framework is used in in robust optimization. It is the strongest from of robustness!} \amy{yes, agreed. it is the strongest form, but too strong, so not necessarily robust in the way you might hope.}
strategies for the outer player.

Given $\outer \in \outerset$, let $\inner^*(\outer) \in \br[\innerset](\outer)$,
and consider an online min-max Stackelberg game $\left\{\left( \outerset, \innerset, \obj[\iter], \constr[][\iter] \right) \right\}$.
In an asymmetric setting, the outer player's regret is the difference between the cumulative loss of their sequence of strategies $\{\outer[][\iter]\}$ (to which the inner player best responds), and the smallest cumulative loss that the outer player could have achieved by playing a fixed strategy $\outer \in \outerset$ (again, to which the inner player best responds), i.e., $\frac{1}{\numiters}\sum_{\iter = 1}^\numiters \obj[\iter](\outer[][\iter], \inner^*(\outer[][\iter])) - \sum_{\iter =1}^\numiters \frac{1}{\numiters} \obj[\iter](\outer, \inner^*(\outer))$. We call this regret the \mydef{asymmetric regret},
%which can be more conveniently defined as the regret incurred by an \samy{action}{strategy} $\outer \in \outerset$ of the outer player w.r.t. a sequence of \samy{actions}{strategies} \sdeni{}{$\{\outer[][\iter]\}_\iter \subset \outerset$} \sdeni{and}{in}\sdeni{ a \sdeni{dynamic}{online} min-max Stackelberg game $\{ \game_\iter \}_{\iter = 1}^\numiters = \left\{(\outerset, \innerset, \obj[\iter], \constr[][\iter]) \right\}_{\iter = 1}^\numiters$ w.r.t. to the}{a} loss given by 
and express it in terms of the outer player's value function $\val[\outerset]$:
%
%\begin{align*}
    $\pesregret[\outerset][\numiters] \left( \left\{ \outer[][\iter] \right\}, \outer \right) = \frac{1}{\numiters}\sum_{\iter = 1}^\numiters \val[\outerset][\iter](\outer[][\iter]) - \sum_{\iter =1}^\numiters \frac{1}{\numiters} \val[\outerset][\iter](\outer)$.
%\enspace .
%\end{align*}
%
\if 0
\noindent
Once again, the outer player's asymmetric regret compares the value achieved by their strategy to the smallest cumulative loss they could have achieved by playing a fixed strategy instead, \emph{assuming the inner player best-responds}. 
%It is \sdeni{}{asymmetric} in the sense that the outer player assumes the worst possible outcome for themself.
%, i.e., the inner player best-responds. 
% Note that for a static min-max Stackelberg game, by the definition of a Stackelberg equilbirium, for $(\outer^*, \inner^*) \in \outerset \times \innerset$, if $\pesregret[\outerset][\numiters](\outer^*) = 0$ and $\inner^* \in \argmax_{\inner \in \innerset: \constr(\outer^*, \inner)} \obj(\outer^*, \inner)$, then $(\outer^*, \inner^*)$ is a $(0,0)$-Stackelberg equilibrium. We call a no-regret algorithm with respect to the \sdeni{pessimistic}{asymmetric} regret a no-\sdeni{pessimistic}{asymmetric}-regret algorithm.
\fi
%
As above, we overload notation and write \\ $\pesregret[\outerset][\numiters] \left( \left\{ \outer[][\iter] \right\} \right) = \max_{\outer \in \outerset} \pesregret[\outerset][\numiters] \left( \left\{ \outer[][\iter] \right\}, \outer \right)$.

The main theorem%
\footnote{The proofs of all mathematical claims in this section can be found in \Cref{sec_app:proofs}.}
in this section states the following: assuming the inner player best responds to the strategies of the outer player, if the outer player employs a no-regret algorithm, then the outer player's average strategy converges to their part of a Stackelberg equilibrium strategy.

% \begin{proposition}[\cite{goktas2021minmax}, Proposition A.1]
% \label{thm:convex-value-func}
% %Suppose that \Cref{main-assum} holds.
% In a min-max Stackelberg game $(\outerset, \innerset, \obj, \constr)$, the outer player's value function, $\val(\outer) = \max_{\inner \in \innerset : \constr(\outer, \inner) \geq \zeros} \obj(\outer, \inner)$, is continuous and convex.
% \end{proposition}

\if 0
\begin{proof}
By Berge's maximum theorem \cite{berge1997topological}, the outer player's value function $\val(\outer) = \max_{\inner \in \innerset: \constr(\outer, \inner) \geq \zeros} \obj(\outer, \inner)$ is continuous.
% , and the inner player's solution correspondence $\innerset^*(\outer) = \argmax_{\inner \in \innerset: \constr(\outer, \inner) \geq \zeros} \obj(\outer, \inner)$ is non-empty, for all $\outer \in \outerset$. 

Let $\lang: \innerset \times \R_+^\numconstrs \times \outerset \to \R$ such that $\lang(\inner, \langmult; \outer) = \obj(\outer, \inner) + \sum_{\numconstr = 1}^\numconstrs \langmult[\numconstr] \constr[\numconstr](\outer, \inner)$ and let $h: \innerset \times \outerset \to \R$ such that $h(\inner; \outer) = \min_{\langmult \in \R_+^\numconstrs} \obj(\outer, \inner) + \sum_{\numconstr = 1}^\numconstrs \langmult[\numconstr] \constr[\numconstr](\outer, \inner)$. We can re-express the outer player's value function via a Lagrangian saddle-point problem which is well defined since Slater's condition holds:
\begin{align}
    \val(\outer) =  \max_{\inner \in \innerset: \constr(\outer, \inner) \geq \zeros} \obj(\outer, \inner) = \max_{\inner \in \innerset} \min_{\langmult \in \R_+^\numconstrs} \lang(\inner, \langmult; \outer) = \max_{\inner \in \innerset} h(\inner; \outer)
\end{align}
Since Slater's condition is satisfied under \Cref{main-assum}, by the KKT theorem \cite{kuhn1951kkt}, we have that for all $\outer \in \outerset, \inner \in \outerset$,  there exists $\langmult^*$ such that $\forall \numconstr \in [\numconstrs],  0 \leq \langmult[\numconstr]^* \leq c < \infty$. We can then re-express the constraint set for the KKT multipliers $\langmult$ such that $\val(\outer) = \max_{\outer \in \outerset} \min_{\langmult \in [0, c]^\numconstrs} \lang(\inner, \langmult; \outer)$. Notice that $\lang$ is convex in $\inner$, concave in $\outer$, and convex in $\langmult$. Since $h$ is the $\inf$-projection of $\lang$ w.r.t. $\langmult$ onto the compact set $[0, c]^\numconstrs$, $h$ must be convex in $\outer$ \cite{rockafellar2009variational}. 
% Additionally, $h$ is concave in $\inner$, since the infimum, or in this case the minimum, of a convex function over a compact index set is convex. \deni{add citation}. 
% Hence, $h$ is convex in $\outer$ and concave in $\inner$.  
Since $\val$ is the supremum, or in this case maximum, of convex functions over a compact index set, i.e., $\max_{\inner \in \innerset} h(\inner; \outer)$, $\val$ is convex.
\end{proof}
\fi

% \amy{define this notation earlier, not in the theorem statements. Write it generically, e.g., for $z$, so that it is meaningful for both $x$ and $y$.
% Let $\avgouter[][\numiters] = \frac{1}{\numiters} \sum_{\iter = 1}^\numiters \outer[][\iter]$.}

% \amy{i think we need to emphasize that the model we are studying is an online min-max Stackelberg game, but in this theorem, we assume the players are playing the same game repeatedly. n'est-ce pas?}\deni{Just adding "repeated" is enough imo.} \amy{precisely, but i was explaining why i added repeated everywhere. to make this distinction!}

\begin{theorem}
\label{thm:pes-regret-bound}
%Suppose that \Cref{main-assum} holds.
Consider a repeated min-max Stackelberg game $(\outerset, \innerset, \obj, \constr)$, and suppose the outer player plays a sequence of strategies $\{\outer[][\iter]\}$. 
% , and that the inner player generates a sequence of best-responses $\{\inner^*(\outer[][\iter])\}_{\iter =1}^\numiters$ such that $\inner^*(\outer[][\iter]) \in \br[\innerset](\outer[][\iter]))$. 
If, after $\numiters$ iterations, the outer player's asymmetric regret is bounded by $\varepsilon$, i.e.,
%for all $\outer \in \outerset$, 
$\pesregret[\outerset][\numiters] \left( \left\{ \outer[][\iter] \right\} \right) \le \epsilon$,
then $\left( \avgouter[][\numiters],  \inner^*(\avgouter[][\numiters]) \right)$ is a $(\varepsilon, 0)$-Stackelberg equilibrium, where $\inner^*(\avgouter[][\numiters]) \in \br[\innerset](\avgouter[][\numiters])$.
% \amy{or: 
% $\max_{\outer \in \outerset} \pesregret[\outerset][\numiters] \left( \left\{ \outer[][\iter] \right\}, \outer \right) \le \epsilon$, if we don't want to overload the notation this way}
\end{theorem}

We remark that although the definition of asymmetric regret looks similar to the standard definition of regret, its structure is very different.
\Cref{thm:convex-value-func} is required to ensure that the time-averaged value function $\sum_{\iter =1}^\numiters \val[][\iter](\outer)$ is convex in $\outer$.

%= \sum_{\iter =1}^\numiters \frac{1}{\numiters} \obj[\iter](\outer, \inner^*(\outer))


\subsection{Symmetric Learning Setting} 

We now turn our attention to a setting in which both players are no-regret learners.
The most straightforward way to define regret is by considering the outer and inner players' ``vanilla'' regrets, respectively: 
%\amy{the regret expressions need more arguments, specifically the x and y sequences.}\deni{Added. The input only is the particular player's sequence of plays. Is that fine? Otherwise it might be too overcrowded if I add the other player's sequence of play as well?}
$\regret[\outerset][\numiters] \left( \{\outer[][\iter]\}, \outer \right) = \frac{1}{\numiters}\sum_{\iter = 1}^\numiters \obj[\iter](\outer[][\iter], \inner[][\iter]) - \frac{1}{\numiters} \sum_{\iter =1}^\numiters  \obj[\iter](\outer, \inner[][\iter])$ and $\regret[\innerset][\numiters] \left( \{\inner[][\iter]\}, \inner \right) = \frac{1}{\numiters} \sum_{\iter =1}^\numiters \obj[\iter](\outer[][\iter], \inner) -  \frac{1}{\numiters}\sum_{\iter = 1}^\numiters \obj[\iter](\outer[][\iter], \inner[][\iter]) $.
In convex-concave min-max games (with independent strategy sets), when both players minimize these regrets, 
%$\regret[\outerset][\numiters]$ and $\regret[\innerset][\numiters]$, respectively
the players' average strategies converge to Nash equilibrium.
In min-max Stackelberg games (with dependent strategy sets), however,
convergence to a Stackelberg equilibrium is not guaranteed.

\begin{example}
Consider the min-max Stackelberg game $\min_{\outer[ ] \in [-1, 1]} \\ \max_{\inner[ ] \in [-1, 1] : 0 \leq 1 - (\outer[ ] + \inner[ ])} \outer[ ]^2 + \inner[ ] + 1$.
The Stackelberg equilibrium of this game is given by $\outer[ ]^* = \nicefrac{1}{2}, \inner[ ]^* = \nicefrac{1}{2}$.

If both players employ no-regret algorithms that generate strategies $\{\outer[][\iter], \inner[][\iter] \}_{\iter \in \N_+}$,
then at time $\numiters \in \N_+$, there exists $\varepsilon > 0$, s.t.
\begin{align*}\left\{
\begin{array}{c}
    \frac{1}{\numiters}\sum_{\iter = 1}^\numiters \left[{\outer[ ][\iter]}^2 + \inner[ ][\iter] + 1 \right]- \frac{1}{\numiters} \min_{\outer[ ] \in [-1, 1]} \sum_{\iter =1}^\numiters \left[\outer[ ]^2 + \inner[ ][\iter] + 1 \right] \leq \varepsilon \\
    \frac{1}{\numiters} \max_{\inner[ ] \in [-1, 1]} \sum_{\iter = 1}^\numiters \left[{\outer[ ][\iter]}^2 + \inner[ ] + 1 \right] -  \frac{1}{\numiters}\sum_{\iter = 1}^\numiters \left[{\outer[ ][\iter]}^2 + \inner[ ][\iter] + 1 \right] \leq \varepsilon  
\end{array}\right.
\end{align*}

\noindent
Simplifying yields:
\begin{align*}
\left\{
\begin{array}{c}
    \frac{1}{\numiters}\sum_{\iter = 1}^\numiters {\outer[ ][\iter]}^2 - \min_{\outer[ ] \in [-1, 1]} \outer[ ]^2 \leq \varepsilon   \\
    \max_{\inner[ ] \in [-1, 1]} \inner[ ] -  \frac{1}{\numiters}\sum_{\iter = 1}^\numiters  \inner[ ][\iter] \leq \varepsilon  
\end{array}\right.
=\left\{
\begin{array}{c}
    \frac{1}{\numiters}\sum_{\iter = 1}^\numiters {\outer[ ][\iter]}^2 \leq \varepsilon \\
    1 - \varepsilon \leq \frac{1}{\numiters}\sum_{\iter = 1}^\numiters  \inner[ ][\iter]
\end{array}\right.
\end{align*}

\if 0
\noindent
Since both players are no-regret learners, there exists $\numiters \in \N_+$ large enough s.t.
%$\varepsilon = 0$:
\begin{align}
\left\{
\begin{array}{c}
    \frac{1}{\numiters}\sum_{\iter = 1}^\numiters {\outer[ ][\iter]}^2   \leq \min_{\outer[ ] \in [-1, 1]} \outer[ ]^2 \\
    \max_{\inner[ ] \in [-1, 1]} \inner[ ]   \leq \frac{1}{\numiters}\sum_{\iter = 1}^\numiters  \inner[ ][\iter]
\end{array}\right.
% \end{align}
% \noindent
% Equivalently,
% \begin{align}
=\left\{
\begin{array}{c}
    \frac{1}{\numiters}\sum_{\iter = 1}^\numiters {\outer[ ][\iter]}^2   \leq 0 \\
    1 \leq \frac{1}{\numiters}\sum_{\iter = 1}^\numiters  \inner[ ][\iter]
\end{array}\right.
\end{align}
\fi

\noindent
In other words, the average iterates converge to $\outer[ ] = 0$, $\inner[ ] = 1$, which is not the Stackelberg equilibrium of this game.
%\samy{Note that this also implies that no-regret learning dynamics does not converge in last iterates.}{} \amy{isn't this obvious? isn't last iterates stronger than average?}
\end{example}

%Note, however, that if the outer player can compute the best-response of the inner player given their \samy{action}{strategy}, then they can instead minimize their \sdeni{pessimistic}{asymmetric} regret, such no-regret learning dynamics will converge to a Stackelberg equilibrium strategy of the outer player in average iterates, but they will not for the inner player because the inner player's strategies are not guaranteed to be feasible.

If the inner player minimizes their vanilla regret without regard to the game's constraints, then their strategies are not guaranteed to be feasible, and thus cannot converge to a Stackelberg equilibrium.
To remedy this infeasibility,
%the infeasibility of the inner player's strategy, 
we introduce a new type of regret we call \mydef{Lagrangian regret}, and show that assuming access to a solution oracle for the optimal KKT multipliers of the game's constraints, if both players minimize their Lagrangian regret, then no-regret learning dynamics converge to a Stackelberg equilibrium.

%For the rest of this paper,
Let $\lang[\outer](\inner, \langmult) = \obj(\outer, \inner) + \sum_{\numconstr = 1}^\numconstrs \langmult[\numconstr] \constr[\numconstr](\outer, \inner)$ denote the Lagrangian associated with the outer player's value function, or equivalently, the inner player's maximization problem, given the outer player's strategy $\outer \in \outerset$.
Using this notation, we can re-express the Stackelberg game as
$\min_{\outer \in \outerset} \max_{\inner \in \innerset : \constr(\outer, \inner) \geq \zeros} \obj(\outer, \inner) = 
%\min_{\outer \in \outerset} \val[\outerset] (\outer) = 
\min_{\outer \in \outerset} \max_{\inner \in \innerset } \min_{\langmult \geq \zeros} \\ \lang[\outer]( \inner, \langmult)$.
If the optimal KKT multipliers $\langmult^* \in \R^\numconstrs$, which are guaranteed to exist 
%under \Cref{main-assum}
by Slater's condition \cite{slater1959convex}, were known, then one could plug them back into the Lagrangian to obtain a convex-concave saddle point problem given by $\min_{\outer \in \outerset} \max_{\inner \in \innerset } \lang[\outer]( \inner, \langmult^*)$.
Note that a saddle point of this problem is guaranteed to exist by the minimax theorem \cite{neumann1928theorie}, since $\lang[\outer]( \inner, \langmult^*)$ is convex in $\outer$ and concave in $\inner$.
%
%Our no-regret learning algorithm in the \sdeni{optimistic}{symmetric} setting relies on
The next lemma states that the Stackelberg equilibria of a min-max Stackelberg game correspond to the saddle points of $\lang[\outer](\inner, \langmult^*)$.

\begin{lemma}
\label{thm:stackelberg-equiv}
%Under \Cref{main-assum}m
Any Stackelberg equilibrium $(\outer^* \inner^*) \in \outerset \times \innerset$ of any min-max Stackelberg game 
%with dependent strategy sets
$(\outerset, \innerset, \obj, \constr)$ corresponds to a saddle point of $\lang[\outer](\inner, \langmult^*)$, where $\langmult^* \in \argmin_{\langmult \geq 0} \min_{\outer \in \outerset} \max_{\inner \in \innerset} \lang[\outer](\inner, \langmult)$.

%Given the outer player's \samy{action}{strategy} $\outer$, let $\lang[\outer](\inner, \langmult) = \obj(\outer, \inner) + \sum_{\numconstr = 1}^\numconstrs \langmult[\numconstr] \constr[\numconstr](\outer, \inner)$ be the Lagrangian associated with the inner player's payoff maximization problem: i.e., $\max_{\inner \in \innerset : \constr(\outer, \inner) \geq \zeros} \obj(\outer, \inner)$.
% can be viewed as a min-max game with independent strategy sets: i.e., \\
% %
% %\begin{align}
% $\min_{\outer \in \outerset} \max_{\inner \in \innerset : \constr(\outer, \inner) \geq \zeros} \obj(\outer, \inner) = \\ \min_{\outer \in \outerset} \max_{\inner \in \innerset } \min_{\langmult \geq \zeros}  \lang[\outer](\inner, \langmult) = \\ \min_{\langmult \geq \zeros, \outer \in \outerset} \max_{\inner \in \innerset } \lang[\outer](\inner, \langmult)$. 
% \sadie{Do we need to fix all the out-of-page here?}\deni{Yes, will have to once I start working on formatting on the AAMAS version :)}\sadie{sure!} \deni{Meanwhile Sadie, you see there is a comment before related works in blue, could you adress that and add more details on what out experiments show there?}\sadie{sure!Let me look at it!}\deni{Thanks!!!}
%\enspace .
%\end{align} 
\end{lemma}

This lemma tells us that the function $\lang[\outer]( \inner, \langmult^*)$ 
%where $\langmult^* \in \argmin_{\langmult \geq 0} \min_{\outer \in \outerset} \max_{\inner \in \innerset} \lang[\outer](\inner, \langmult)$
represents a new loss function that enforces the game's constraints.
%$\constr$.
Based on this observation, we assume access to a Lagrangian solution oracle that provides us with $\langmult^* \in \argmin_{\langmult \geq 0} \min_{\outer \in \outerset} \max_{\inner \in \innerset} \lang[\outer](\inner, \langmult^*)$.

Next, we define a new type of regret which we call \mydef{Lagrangian regret}.
Given a sequence of strategies $\left\{\outer[][\iter], \inner[][\iter]\right\}$ played by the outer and inner players in an online min-max Stackelberg game $\left\{ \left( \outerset, \innerset, \obj[\iter], \constr[][\iter] \right) \right\}$, we define their Lagrangian regret, respectively, as $\langregret[\outerset][\numiters] \left( \left\{ \outer[][\iter] \right\}, \outer \right) = \frac{1}{\numiters}\sum_{\iter = 1}^\numiters \lang[{\outer[ ][\iter]}][\iter](\inner[][\iter], \langmult^*) - \frac{1}{\numiters} \sum_{\iter =1}^\numiters  \lang[\outer][\iter] (\inner[][\iter],\langmult^*)$ and $\langregret[\innerset][\numiters] \left( \left\{ \inner[][\iter] \right\}, \inner \right) = \frac{1}{\numiters} \sum_{\iter =1}^\numiters \lang[{\outer[][\iter]}][\iter](\inner, \langmult^*) -  \frac{1}{\numiters}\sum_{\iter = 1}^\numiters \lang[{\outer[][\iter]}][\iter](\inner[][\iter], \langmult^*)$. 
We further define $\langregret[\outerset][\numiters] \left( \left\{ \outer[][\iter] \right\}\right)$ and $\langregret[\innerset][\numiters] \left( \left\{ \inner[][\iter] \right\}\right)$ as expected.
%\sdeni{}{For notational simplicity we also denote $\langregret[\outerset][\numiters] \left( \left\{ \outer[][\iter] \right\}\right) = \max_{\outer \in \outerset} \langregret[\outerset][\numiters] \left( \left\{ \outer[][\iter] \right\}, \outer \right)$, and $\langregret[\innerset][\numiters] \left( \left\{ \inner[][\iter] \right\}\right) = \max_{\inner \in \innerset} \langregret[\innerset][\numiters] \left( \left\{ \inner[][\iter] \right\}, \inner \right)$.}

The \mydef{saddle point residual} of a point $(\outer^*, \inner^*) \in \outerset \times \innerset$ w.r.t.{} a convex-concave function $h: \outerset \times \innerset \to \R$ is given by $\max_{\inner \in \innerset} h(\outer^*, \inner) - \min_{\outer \in \outerset} h(\outer, \inner^*)$.
When the saddle point residual of $(\outer, \inner)$ w.r.t. $\lang[\outer](\inner, \langmult^*)$ is 0, %\sadie{Also, $\lang[\outer](\inner, \langmult^*)$ only takes $y$ as input but not $x$, is this a problem?}\deni{To me it's not an issue because any other notation just makes it more cumbersome.}
the saddle point is a $(0, 0)$-Stackelberg equilibrium.

The main theorem of this section now follows: if both players play so as to minimize their Lagrangian regret, then their average strategies converge to a Stackelberg equilibrium. 
The bound is given in terms of the saddle point residual of the iterates generated.
%\amy{same question as above.}\sadie{"saddle point with respect to $\lang[\outer](\inner, \langmult^*)$"?}

\begin{theorem}
\label{thm:lang-regret-bound}
%Suppose \Cref{main-assum} holds.
Consider a repeated min-max Stackelberg game $(\outerset, \innerset, \obj, \constr)$, and suppose the outer and the players generate sequences of strategies $\{(\outer[][\iter], \inner[][\iter])\}$ using a no-Lagrangian-regret algorithm.
% , and that the inner player generates a sequence of best-responses $\{\inner^*(\outer[][\iter])\}_{\iter =1}^\numiters$ such that $\inner^*(\outer[][\iter]) \in \br[\innerset](\outer[][\iter]))$.
If after $\numiters$ iterations, the Lagrangian regret of both players is bounded by $\varepsilon$, i.e., 
$\langregret[\outerset][\numiters] \left( \left\{ \outer[][\iter] \right\} \right) \le \varepsilon$ and
$\langregret[\innerset][\numiters] \left( \left\{ \inner[][\iter] \right\} \right) \le \epsilon$,
then the following convergence bound holds on the saddle point residual of $(\avgouter[][\numiters], \avginner[][\numiters])$ w.r.t.\ the Lagrangian:
%\begin{align}
    $0 \leq \max_{\inner \in \innerset}  \lang[{\avgouter[][\numiters]}](\inner, \langmult^*) - \min_{\outer \in \outerset}  \lang[\outer] (\avginner[][\numiters],\langmult^*) \leq 2\varepsilon$.
%\end{align}
\end{theorem}

\if 0
% \amy{i think these are the wrong references. there are no corollaries in this section:}
We remark that, unlike the result in \Cref{thm:pes-regret-bound}, which provides a convergence bound 
%to an approximate 
in terms of a Stackelberg equilibrium residual, \Cref{thm:lang-regret-bound} provides a convergence bound in terms of the saddle point residual of the Lagrangian.
\fi

Having provided convergence to Stackelberg equilibrium of general no-regret learning dynamics in repeated min-max Stackelberg games, we now proceed to investigate the convergence and robustness properties of a specific example of a no-regret learning dynamic, namely online mirror descent (OMD).


==> Robust No-Regret Learning in Min Max Stackelberg Games (AAMAS 2022)/conclusion.tex <==
\section{Conclusion}

We began this paper by considering no-regret learning dynamics in repeated min-max Stackelberg games in two settings: an asymmetric setting in which the outer player is a no-regret learner and the inner player best responds, and a {symmetric} setting in which both players are no-regret learners.
For both of these settings, we proved that no-regret learning dynamics converge to a Stackelberg equilibrium of the game.
We then specialized the no-regret algorithm employed by the players to online mirror descent (OMD), which yielded two new algorithms, max-oracle MD and nested MDA in the asymmetric setting, and a new simultaneous GDA-like algorithm \cite{nedic2009gda}, which we call Lagrangian MDA, in the symmetric setting.
As these algorithms are no-regret learning algorithms, our earlier theorems imply convergence to $\varepsilon$-Stackelberg equilibria in $O(\nicefrac{1}{\varepsilon^2})$ iterations for max-oracle MD and LMDA, and $O(\nicefrac{1}{\varepsilon^3})$ iterations for nested MDA.

Finally, as many real-world applications involve changing environments, we investigated the robustness of OMD dynamics by analyzing how closely they track Stackelberg equilibria in arbitrary online min-max Stackelberg games.
We proved that in min-max games (with independent strategy sets) OMD dynamics closely track the changing Stackelberg equilibria of a game.
As we were not able to extend these theoretical robustness guarantees to min-max Stackelberg games (with dependent strategy sets), we instead ran a series of experiments with online Fisher markets, which are canonical examples of min-max Stackelberg games.
Our experiments suggest that OMD dynamics are robust for min-max Stackelberg games so that perhaps the robustness guarantees we have provided for OMD dynamics in min-max games (with independent strategy sets) can be extended to min-max Stackelberg games (with dependent strategy sets). 

The theory developed in this paper opens the door to extending the myriad applications of Stackelberg games in AI to incorporating dependent strategy sets.
Such models promise to be more expressive, and as a result could provide decision makers with better solutions to problems in security, environmental protection, etc.
%, ranging from fairness in machine learning to generative adversarial learning to security games.


==> Robust No-Regret Learning in Min Max Stackelberg Games (AAMAS 2022)/fisher.tex <==
\section{Online Fisher Markets}
\label{sec:experiments}

\if 0
\begin{algorithm}[H]
\caption{GDA with solution oracle}
\label{alg:myopic-br}
\textbf{Inputs:} $\util, \budget, \learnrate[][\price], \learnrate[][\allocation], \iters, \allocation^{(0)}, \price^{(0)}$ \\ 
\textbf{Output:} $\outer^{*}, \inner^{*}$
\begin{algorithmic}[1]
\For{$\iter = 1, \hdots, \iters -1$}
    \State Set $\price^{(\iter +1)} = \project[\R_+^\numgoods] \left( \ones[\numgoods] - \sum_{\buyer \in \buyers} \allocation[\buyer]^{(t)} \right)$
    \State For all $\buyer \in \buyers$, set $\allocation[\buyer]^{(\iter +1)} = \project[\{{ \allocation[ ] \in 
    \R^\numgoods_+ : \allocation[ ] \cdot \price^{(\iter-1)} \leq \budget[\buyer]^{(\iter)}}\}] \left( \allocation[\buyer]^{(\iter)} + \learnrate[\iter][\inner]  \frac{\budget[\buyer]^{(\iter)}}{\util[\buyer]^{(\iter)}\left(\allocation[\buyer]^{(\iter)}\right)} \grad[{\allocation[\buyer]}] \util[\buyer]^{(\iter)}\left(\allocation[\buyer]^{(\iter)}\right) \right)$
\EndFor
% \State Draw $(\widehat{\price}, \widehat{\allocation})$ uniformly at random from $\{(\price^{(\iter)}, \allocation^{(\iter)}\}_{\iter = 1}^\iters$
\State \Return $(\price^{(\iter)}, \allocation^{(\iter)})_{\iter = 1}^\iters$ 
\end{algorithmic}
\end{algorithm}
\fi

The Fisher market model, attributed to Irving Fisher \cite{brainard2000compute}, has received a great deal of attention in the literature, especially by computer scientists, as it has proven useful in the design of electronic marketplaces.
We now study OMD dynamics in online Fisher markets, which are instances of min-max Stackelberg games \cite{goktas2021minmax}.

A \mydef{Fisher market} consists of $\numbuyers$ buyers and $\numgoods$ divisible goods \cite{brainard2000compute}.
Each buyer $\buyer \in \buyers$ has a budget $\budget[\buyer] \in \mathbb{R}_{+}$ and a utility function $\util[\buyer]: \mathbb{R}_{+}^{\numgoods} \to \mathbb{R}$.
%\footnote{\sdeni{WLOG, we assume that all budgets are strictly positive; otherwise, we could remove a buyer with a zero budget without affecting the equilibrium.}{}} 
Each good $\good \in \goods$ has supply $\supply[\good] \in \R_+$.
A Fisher market is thus given by a tuple $(\numbuyers, \numgoods, \util, \budget, \supply)$, where $\util = \left\{\util[1], \hdots, \util[\numbuyers] \right\}$ is a set of utility functions, one per buyer; $\budget \in \R_{+}^{\numbuyers}$ is a vector of buyer budgets; and $\supply \in \R^\numgoods_+$ is a vector of good supplies.
We abbreviate as $(\util, \budget, \supply)$ when $\numbuyers$ and $\numgoods$ are clear from context.
An \mydef{online Fisher market} is a sequence of Fisher markets $\left\{\left( \util^{(\iter)}, \budget^{(\iter)}, \supply^{(\iter)} \right)\right\}_{\iter = 1}^{\numiters}$.
%, possibly varying over time.
%which describe a Fisher market that changes across time. 

An \mydef{allocation} $\allocation = \left(\allocation[1], \hdots, \allocation[\numbuyers] \right)^T \in \R_+^{\numbuyers \times \numgoods}$ is an assignment of goods to buyers, represented as a matrix s.t.\ $\allocation[\buyer][\good] \ge 0$ denotes the amount of good $\good \in \goods$ allocated to buyer $\buyer \in \buyers$.
Goods are assigned \mydef{prices} $\price = \left(\price[1], \hdots, \price[\numgoods] \right)^T \in \mathbb{R}_+^{\numgoods}$.
A tuple $(\price^*, \allocation^*)$ is said to be a \mydef{competitive 
%(or Walrasian)
equilibrium (CE)} of Fisher market $(\util, \budget, \supply)$ if 1.~buyers are utility maximizing, constrained by their budget, i.e., $\forall \buyer \in \buyers, \allocation[\buyer]^* \in \argmax_{\allocation[ ] : \allocation[ ] \cdot \price^* \leq \budget[\buyer]} \util[\buyer](\allocation[ ])$;
and 2.~the market clears, i.e., $\forall \good \in \goods,  \price[\good]^* > 0 \Rightarrow \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^* = \supply[\good]$  and $\price[\good]^* = 0 \Rightarrow\sum_{\buyer \in \buyers} \allocation[\buyer][\good]^* \leq \supply[\good]$.

\citeauthor{goktas2021minmax} \cite{goktas2021minmax} observe that any CE $(\price^*, \allocation^*)$ of a Fisher market $(\util, \budget)$ corresponds to a Stackelberg equilibrium of the following min-max Stackelberg game:%
\footnote{The first term in this program is slightly different than the first term in the program presented by \citeauthor{goktas2021minmax} \cite{goktas2021minmax}, since supply is assumed to be 1 their work.}
%
\begin{align}
    \min_{\price \in \R_+^\numgoods} \max_{\allocation \in \R^{\numbuyers \times \numgoods}_+ :  \allocation \price \leq \budget} \sum_{\good \in \goods} \supply[\good] \price[\good] + \sum_{\buyer \in \buyers}  \budget[\buyer] \log \left(  \util[\buyer](\allocation[\buyer]) \right) \enspace .
    \label{fisher-program}
\end{align}

\noindent
Let $\lang: \R^\numgoods_+ \times \R^{\numbuyers \times \numgoods} \to \R_+$ be the Lagrangian of the outer player's value function in \Cref{fisher-program}, i.e., 
$\lang[\price](\allocation, \langmult) = \sum_{\good \in \goods} \supply[\good] \price[\good] \\ + \sum_{\buyer \in \buyers}  \budget[\buyer] \log \left(  \util[\buyer](\allocation[\buyer]) \right) + \sum_{\buyer \in \buyers} \langmult[\buyer] \left( \budget[\buyer] - \allocation[\buyer] \cdot \price \right)$. One can show the existence of a Lagrangian solution oracle for the Lagrangian of \Cref{fisher-program} such that $\langmult^* = \ones[\numgoods]$. 
We then have: 1.~ by \citeauthor{goktas2021minmax}'s envelope theorem, the subdifferential of the outer player's value function is given by $\grad[\price] \val(\price) = \supply - \sum_{\buyer \in \buyers} \allocation[\buyer]^*(\price)$, where $\allocation[\buyer]^*(\price) \in \argmax_{\allocation[ ] \in \R^\numgoods_+ \allocation[ ] \cdot \price \leq \budget[\buyer]} \util[\buyer](\allocation[ ])$, 2.~the gradient of the Lagrangian w.r.t. the prices, given the Lagrangian solution oracle, is $\grad[\price] \lang[\price](\allocation, \langmult^*) = \supply - \sum_{\buyer \in \buyers} \allocation[\buyer]$  
and
$\grad[{\allocation[\buyer]}] \lang[\price](\allocation, \langmult^*)) = \frac{\budget[\buyer]}{\util[\buyer]\left(\allocation[\buyer]\right)} \grad[{\allocation[\buyer]}] \util[\buyer]\left(\allocation[\buyer]\right) - \price$, 
where $\langmult^* = \ones[\numgoods]$ \cite{goktas2021consumer}. 
%\sadie{Do we need to state that $\langmult^*(\allocation^*(\price), \price) = \ones[\numgoods]$ as a corollary?}\deni{Good question, what do you think Amy?}

% At each time step $\iter$, we have a problem of computing a competitive equilibrium $(\price^{(\iter)^*}, \allocation^{(\iter)^*})$ of a Fisher market $(\util^{(\iter)}, \budget^{(\iter)}, \supply^{(\iter)})$, where $\util^{(\iter)}$ is a set of continuous, concave, and homogeneous\sadie{I don't know whether we can relax this condition}\deni{We can't!} utility functions.
% This problem can be solved via the Eisenberg-Gale convex program  \cite{eisenberg1959consensus}, and it allows us to compute the distance between our dynamic and the competitive equilibrium, which can be considered as a Stackelberg equilibrium in the min-max game setting, at each time period. 

We first consider OMD dynamics for Fisher markets in the asymmetric setting, in which the outer player determines their strategy via projected OGD {first} and the inner player best-responds. 
% Noting that $\grad[\price] \lang[\price](\allocation^*, \langmult^*(\allocation^*(\price), \price)) = \supply - \sum_{\buyer \in \buyers} \allocation[\buyer]$,
% \citeauthor{goktas2021minmax}, 
This setup yields a dynamic version of a natural price adjustment process known as t\^atonnement \cite{walras}, this variant of which
% \amy{it sounded like t\^atonnement itself was first studied by Cheung}
was first studied by \citeauthor{cheung2019tracing} \cite{cheung2019tracing} (\Cref{alg:dynamic_max_oracle_gd}, \Cref{sec-app:algos}). 

% \begin{algorithm}[H]
% \caption{Max-Oracle Gradient Descent}
% \label{alg:max_oracle_gd}
% \textbf{Inputs:} $\util, \budget, \supply, \learnrate, \iters,  \price^{(0)}, \delta$ \\ 
% \textbf{Output:} $\outer^{*}, \inner^{*}$
% \begin{algorithmic}[1]
% \For{$\iter = 1, \hdots, \iters -1$}
%     \State For all $\buyer \in \buyers$, find $\allocation[\buyer]^{(t)}$ s.t. $\util[\buyer](\allocation[\buyer]^{(\iter)} \geq \max_{\allocation[\buyer]:\allocation[\buyer]\cdot \price^{(\iter-1)} \leq \budget[\buyer]}
%     \util[\buyer](\allocation[\buyer]) - \delta$
%     and $\allocation[\buyer]^{(\iter-1)} \cdot \price^{(\iter-1)} \leq \budget[\buyer]$
%     \State Set $\price^{(\iter)}
%     =\project[\R_+^\numgoods]\left(
%     \price^{(t-1)} - \learnrate[t](\supply - \sum_{\buyer \in \buyers} \allocation[\buyer]^{(t)})
%     \right)$
% \EndFor
% \State \Return $(\price^{(\iter)}, \allocation^{(\iter)})_{\iter = 1}^\iters$ 
% \end{algorithmic}
% \end{algorithm}

We also consider OMD dynamics in the {symmetric} setting, specifically the case in which both the outer and inner players employ projected OGD {simultaneously}, which yields myopic best-response dynamics \cite{monderer1996potential} (\Cref{alg:dynamic_lgda}, \Cref{sec-app:algos}).
In words, 
%under myopic best-response dynamics, 
at each time step, the (fictional Walrasian) auctioneer takes a gradient descent step to minimize its regret, and then all the buyers take a gradient ascent step to minimize their Lagrangian regret.
These GDA dynamics can be seen as myopic best-response dynamics for boundedly rational 
%\cite{camerer1998bounded} 
sellers and buyers.

% \begin{algorithm}[H]
% \caption{LGDA}
% \label{alg:lgda}
% \textbf{Inputs:} $\util, \budget, \supply, \learnrate[][\price], \learnrate[][\allocation], \iters, \allocation^{(0)}, \price^{(0)}$ \\ 
% \textbf{Output:} $\outer^{*}, \inner^{*}$
% \begin{algorithmic}[1]
% \For{$\iter = 1, \hdots, \iters -1$}
%     \State Set $\price^{(\iter +1)} = \project[\R_+^\numgoods] \left( \ones[\numgoods] - \sum_{\buyer \in \buyers} \allocation[\buyer]^{(t)} \right)$ 
%     \sadie{Should this be $\project[\R_+^\numgoods]\left(
%     \price^{(t)} - \learnrate[t][\outer](\supply - \sum_{\buyer \in \buyers} \allocation[\buyer]^{(t)})
%     \right)$?}
%     \State For all $\buyer \in \buyers$, set $\allocation[\buyer]^{(\iter +1)} = \project[\R^\numgoods_+] \left( \allocation[\buyer]^{(\iter)} + \learnrate[\iter][\inner]  \left( \frac{\budget[\buyer]^{(\iter)}}{\util[\buyer]^{(\iter)}\left(\allocation[\buyer]^{(\iter)}\right)} \grad[{\allocation[\buyer]}] \util[\buyer]^{(\iter)}\left(\allocation[\buyer]^{(\iter)}\right) - \price^{(\iter)} \right)\right)$
% \EndFor
% % \State Draw $(\widehat{\price}, \widehat{\allocation})$ uniformly at random from $\{(\price^{(\iter)}, \allocation^{(\iter)}\}_{\iter = 1}^\iters$
% \State \Return $(\price^{(\iter)}, \allocation^{(\iter)})_{\iter = 1}^\iters$ 
% \end{algorithmic}
% \end{algorithm}

\paragraph{Experiments}

In order to better understand the robustness properties of Algorithms~\ref{alg:dynamic_max_oracle_gd} and~\ref{alg:dynamic_lgda} in an {online} min-max Stackelberg game that is subject to perturbation across time, we ran a series of experiments with {online} Fisher Markets assuming three different classes of utility functions.%
\footnote{Our code can be found at \coderepo.}
Each utility structure endows \Cref{fisher-program} with different smoothness properties, which allows us to compare the efficiency of the algorithms under varying conditions.
Let $\valuation[\buyer] \in \R^\numgoods$ be a vector of valuation parameters that describes the utility function of buyer $\buyer \in \buyers$.
We consider the following utility function classes:
1.~linear: $\util[\buyer](\allocation[\buyer]) = \sum_{\good \in \goods} \valuation[\buyer][\good] \allocation[\buyer][\good]$; 2.~Cobb-Douglas:  $\util[\buyer](\allocation[\buyer]) = \prod_{\good \in \goods} \allocation[\buyer][\good]^{\valuation[\buyer][\good]}$; and 3.~Leontief:  $\util[\buyer](\allocation[\buyer]) = \min_{\good \in \goods} \left\{ \frac{\allocation[\buyer][\good]}{\valuation[\buyer][\good]}\right\}$.

To simulate an {online} Fisher market, we fix a range for every market parameter and draw from that range uniformly at random during each iteration.
Our goal is to understand how closely OMD dynamics track the CE of the Fisher markets as they vary with time.
We compare the iterates $\left(\price^{(\iter)}, \allocation^{(\iter)} \right)$ computed by the algorithms and the CE $\left(\price^{(\iter)^{*}}, \allocation^{(\iter)^{*}} \right)$ of the market $(\util^{(\iter)}, \budget^{(\iter)}, \supply^{(\iter)})$ at each iteration $\iter$.
The difference between these outcomes is measured as $\left\| {\price^{(\iter)^{*}} - \price^{(\iter)}} \right\|_2 + \left\| {\allocation^{(\iter)^{*}} - \allocation^{(\iter)}} \right\|_2$.

\begin{figure*}
  \begin{minipage}[c]{0.625\textwidth}
    \includegraphics[width=\textwidth]{graphs/gd_pplusx_dist_graphs_random.jpg}
  \end{minipage}\hfill
  \begin{minipage}[c]{0.33\textwidth}
    \caption{In {\color{blue} blue}, we depict a trajectory of distances between computed allocation-price pairs and equilibrium allocation-price pairs, when \Cref{alg:dynamic_max_oracle_gd} is run on randomly initialized online linear, Cobb-Douglas, and Leontief Fisher markets. In {\color{red} red}, we plot an arbitrary $O(\nicefrac{1}{\sqrt{T}})$ function.}
    \label{fig:exp_results_gd}
  \end{minipage}
%
  \begin{minipage}[c]{0.625\textwidth}
    \includegraphics[width=\textwidth]{graphs/lgda_pplusx_dist_graphs_random.jpg}
  \end{minipage}\hfill
  \begin{minipage}[c]{0.33\textwidth}
    \caption{In {\color{blue} blue}, we depict a trajectory of distances between computed allocation-price pairs and equilibrium allocation-price pairs, when \Cref{alg:dynamic_lgda} is run on randomly initialized online linear, Cobb-Douglas, and Leontief Fisher markets. In {\color{red} red}, we plot an arbitrary $O(\nicefrac{1}{\sqrt{T}})$ function.}
    \label{fig:exp_results_lgda}
  \end{minipage}
\end{figure*}

In our experiments, we ran Algorithms~\ref{alg:dynamic_max_oracle_gd} and~\ref{alg:dynamic_lgda} on 100 randomly initialized {online} Fisher markets.
We depict the distance to the CE at each iteration for a single experiment chosen at random in Figures~\ref{fig:exp_results_gd} and~\ref{fig:exp_results_lgda}.
In these figures, we observe that the OMD dynamics are closely tracking the CE as they vary with time.
%, as shown by the overall decreasing distance to equilibrium.
A more detailed description of our experimental setup can be found in \Cref{sec-app:fisher}.
 
We observe from Figures~\ref{fig:exp_results_gd} and~\ref{fig:exp_results_lgda} that for both Algorithms~\ref{alg:dynamic_max_oracle_gd} and~\ref{alg:dynamic_lgda}, we obtain an empirical convergence rate relatively close to $O(\nicefrac{1}{\sqrt{T}})$ under Cobb-Douglas utilities, and a slightly slower empirical convergence rate under linear utilities.
Recall that $O(\nicefrac{1}{\sqrt{T}})$ is the convergence rate guarantee we obtained for both algorithms, assuming a fixed learning rate in a repeated Fisher market  (Corollaries~\ref{corr:max-oracle-gradient-descent} and~\ref{cor:simu-omd}).
%Although our theoretical convergence rate of $O(\nicefrac{1}{\sqrt{T}})$ (Corollaries~\ref{corr:max-oracle-gradient-descent} and~\ref{cor:simu-omd}) applies to (static) Fisher markets with linear and Cobb-Douglas utilities, these results still make sense because the $O(\nicefrac{1}{\sqrt{T}})$ bound is based on fixed learning rates set for a static market. 
Our theoretical results assume fixed learning rates, but since those results apply to repeated games while our experiments apply to {online} Fisher markets, we selected variable learning rates. 
After manual hyper-parameter tuning, for \Cref{alg:dynamic_max_oracle_gd}, we chose a dynamic learning rate of $\learnrate[\iter][ ] = \frac{1}{\sqrt{\iter}}$, while for \Cref{alg:dynamic_lgda}, we chose learning rates of $\learnrate[\iter][\outer] = \frac{5}{\sqrt{\iter}}$ and $\learnrate[\iter][\inner] = \frac{0.01}{\sqrt{\iter}}$, for all $\iter \in \iters$.
For these optimized learning rates, we obtain empirical convergence rates close to what the theory predicts.
%  We also observe that the convergence curve for dynamic Fisher market with linear utility is not very smooth, and this may be attributed to the fact that the value function under linear utility is not differentiable. \sadie{Not pretty sure here.}
 
In Fisher markets with Leontief utilities, the objective function is not differentiable.
Correspondingly, {online} Fisher markets with Leontief utilities are the hardest markets of the three for our algorithms to solve. 
Still, we only see a slightly slower than $O(\nicefrac{1}{\sqrt{T}})$ empirical convergence rate.
%For \sdeni{dynamic}{online} Fisher markets with Leontief utilities,
In these experiments, the convergence curve generated by \Cref{alg:dynamic_lgda} has a less erratic behavior than the one generated by \Cref{alg:dynamic_max_oracle_gd}.
Due to the non-differentiability of the objective function, the gradient ascent step in \Cref{alg:dynamic_lgda} for buyers with Leontief utilities is very small, 
% and similarly for linear utilities the gradient descent step ends up being very small due to non-differentiability of the value function of the outer player. This 
effectively dampening any potentially erratic changes in the iterates. 
 
% Considering that the value function is not differentiable assuming linear utilities and objective functions is not differentiable assuming Leontief utilities, our experiment results suggests that differentiability of the value function and objective function is not essential to guarantee convergence of our OMD dynamics. 

Our experiments suggest that OMD dynamics (Algorithms~\ref{alg:dynamic_max_oracle_gd} and \ref{alg:dynamic_lgda}) are robust enough to closely track the changing CE in {online} Fisher markets.
We note that  t\^atonnement dynamics (\Cref{alg:dynamic_max_oracle_gd}) seem to be more robust than myopic best response dynamics (\Cref{alg:dynamic_lgda}), i.e., the distance to equilibrium allocations is smaller at each iteration of t\^atonnement.
This result is not surprising, as t\^atonnement computes a utility-maximizing allocation for the buyers at each time step.
Even though Theorems~\ref{thm:robustness_gd} and~\ref{thm:robustness_lgda} only provide theoretical guarantees on the robustness of OMD dynamics in online min-max games (with independent strategy sets), it seems that similar theoretical robustness results may be attainable in online min-max Stackelberg games (with dependent strategy sets). 


==> Robust No-Regret Learning in Min Max Stackelberg Games (AAMAS 2022)/intro.tex <==
\section{Introduction}
\label{sec:intro}

Min-max optimization problems (i.e., zero-sum games) have been attracting a great deal of attention recently because of their applicability to problems in fairness in machine learning \cite{dai2019kernel, edwards2016censoring, madras2018learning, sattigeri2018fairness}, generative adversarial imitation learning \cite{cai2019global, hamedani2018iteration}, reinforcement learning \cite{dai2018rl}, generative adversarial learning \cite{sanjabi2018convergence}, \amy{you should cite Goodfellow here. wasn't it his idea originally?} adversarial learning \cite{sinha2020certifying}, and statistical learning, e.g., learning parameters of exponential families \cite{dai2019kernel}. 
%
These problems are often modelled as \mydef{min-max games}, i.e., constrained min-max optimization problems of the form:
$\min_{\outer \in \outerset} \max_{\inner \in \innerset} \obj(\outer, \inner)$,
where $\obj: \outerset \times \innerset \to \R$ is continuous, and $\outerset \subset \R^\outerdim$ and $\innerset \subset \R^\innerdim$ are non-empty and compact.
In \mydef{convex-concave min-max games}, where $\obj$ is convex in $\outer$ and concave in $\inner$, von Neumann and Morgenstern's seminal minimax theorem holds  \cite{neumann1928theorie}: i.e.,
$\min_{\outer \in \outerset} \max_{\inner \in \innerset} \obj(\outer, \inner) = \max_{\inner \in \innerset} \min_{\outer \in \outerset} \obj(\outer, \inner)$, guaranteeing the existence of a saddle point, i.e., a point that is simultaneously a minimum of $\obj$ in the $\outer$-direction and a maximum of $\obj$ in the $\inner$-direction.
Because of the minimax theorem, we can interpret the constrained optimization problem as a simultaneous-move, zero-sum game, where $\inner^*$ (resp. $\outer^*$) is a best-response of the outer (resp. inner) player to the other's action $\outer^*$ (resp. $\inner^*)$, in which case a saddle point is also called a minimax point or a Nash equilibrium.

In this paper, we study %no-regret learning dynamics in
\mydef{min-max Stackelberg games} \cite{goktas2021minmax}, i.e., constrained min-max optimization problems \emph{with dependent feasible sets\/} of the form: $\min_{\outer \in \outerset} \max_{\inner \in \innerset : \constr(\outer, \inner) \geq \zeros} \obj(\outer, \inner)$,
where $\obj: \outerset \times \innerset \to \R$ is continuous, $\outerset \subset \R^\outerdim$ and $\innerset \subset \R^\innerdim$ are non-empty and compact, and $\constr(\outer, \inner) = \left(\constr[1](\outer, \inner), \hdots, \constr[\numconstrs](\outer, \inner) \right)^T$ with $\constr[\numconstr]: \outerset \times \innerset \to \R$.
\citeauthor{goktas2021minmax} observe that the minimax theorem does not hold in these games \cite{goktas2021minmax}.
%\footnote{When a Nash equilibrium exists in a min-max Stackelberg game, the game reduces to a simultaneous-move game and the Stackelberg equilibrium of the game coincides with the Nash.}
As a result, such games are more appropriately viewed as sequential, i.e., Stackelberg, games for which the relevant solution concept is the Stackelberg equilibrium,%
\footnote{Alternatively, one could view such games as pseudo-games (also known as abstract economies) \cite{arrow-debreu}, in which players move simultaneously under the unreasonable assumption that the moves they make will satisfy the game's dependency constraints.
Under this view, the relevant solution concept is generalized Nash equilibrium \cite{facchinei2007generalized, facchinei2010generalized}.}
where the outer player chooses $\hat{\outer} \in \outerset$ before the inner player responds with their choice of $\inner(\hat{\outer}) \in \innerset$ s.t.\ $\constr(\hat{\outer}, \inner(\hat{\outer})) \geq \zeros$.
%\footnote{\sdeni{Note that this use of the term value function in economics is distinct from its use in reinforcement learning.}{} \amy{why cross this out?}\deni{Seems obvious but if you disagree let's keep it, we just have a lot of footnotes!}}
%In these games, the outer player seeks to minimize their loss assuming the inner player best responds.
The outer player's objective, which is referred to as their \mydef{value function} in the economics literature \cite{milgrom2002envelope} and which they seek to minimize, is defined as $\val[\outerset](\outer) = \max_{\inner \in \innerset : \constr(\outer, \inner) \geq \zeros} \obj(\outer, \inner)$.
The inner player's value function, $\val[\innerset]: \outerset \to \R$, which they seek to maximize, is simply the objective function of the game, given the outer player's action $\hat{\outer}$: i.e., $\val[\innerset](\inner; \hat{\outer}) = \obj(\hat{\outer}, \inner)$.
%\amy{might want to use the $\hat{\outer}$ notation elsewhere as well.}

\if 0
An important issue at the heart of algorithmic game theory, is understanding learning processes by which players of a game can reach an equilibrium when the game is played in a repeated fashion. One effective way in which players can decide strategies to play in this repeated setting is by minimizing their regret, i.e., by playing a fixed action which minimizes the loss incurred by the player in hindsight. When a player decides their strategies so as to minimize their regret, achieving an average regret of zero as the game is played infinitely, the player is said to be a no-regret learner and their learning process is called a no-regret learning dynamic. 
\fi

\citeauthor{goktas2021minmax} \cite{goktas2021minmax} proposed a polynomial-time first-order method by which to compute Stackelberg equilibria, which they called \mydef{nested gradient descent ascent (GDA)}.
%, consisting of two nested gradient evaluation loops.
This method can be understood as an algorithm a third party might run to find an equilibrium, or as a game dynamic that the players might employ if their long-run goal were to reach an equilibrium.
Rather than assume that players are jointly working towards the goal of reaching an equilibrium, it is often more reasonable to assume that they play so as to not regret their decisions: i.e., that they employ a \mydef{no-regret learning algorithm}, which minimizes their loss in hindsight.
It is well known that when both players in a repeated min-max game are no-regret learners, the players' strategy profile over time converges to a Nash equilibrium in average iterates: i.e., 
%\sdeni{the players' joint}{}\deni{why joint? its technically marginal empirical play distribution, no?}
empirical play converges to a Nash equilibrium (e.g., \cite{freund1996game}).

% \input{related}

In this paper, we investigate no-regret learning dynamics in repeated min-max Stackelberg games.
We assume both an asymmetric and a symmetric setting.
In the asymmetric setting, the outer player is a no-regret learner while the inner player best responds; in the symmetric setting, both players are no-regret learners.
In the asymmetric case, we show that if the outer player uses a no-regret algorithm that achieves $\varepsilon$-{asymmetric} regret, then the outer player's empirical play converges to their $\varepsilon$-Stackelberg equilibrium strategy.
%in average iterates.
%\footnote{We use the notion of an $\varepsilon$-Stackelberg equilibrium loosely in this section.  A precise definition appears later.} 
In the symmetric case, we introduce a new type of regret, which we call Lagrangian regret,%
%\deni{Should we cite the paper the reviewer had mentioned}\amy{only if there is space to do so} 
%%% SPACE
\footnote{We note that similar notions of Lagrangian regret have been used in other online learning settings (e.g., \cite{bechavod2020metric}), but to our knowledge, ours is the first game-theoretic analysis of Lagrangian regret minimization.}
which assumes access to a solution oracle for the optimal KKT multipliers of the game's constraints.
We then show that if both players use no-regret algorithms that achieve $\varepsilon$-Lagrangian regrets, then the players' empirical play converges to an $\varepsilon$-Stackelberg equilibrium.
%in average iterates.

Next, we restrict our attention to a specific no-regret dynamic, namely online mirror descent (OMD)~\cite{nemirovski2004prox}.
Doing so yields two algorithms, max-oracle mirror descent (max-oracle MD) and nested mirror descent ascent (nested MDA) in the asymmetric setting, and a new simultaneous GDA-like algorithm \cite{nedic2009gda} in the symmetric setting, which we call Lagrangian mirror descent ascent (LMDA).
The first two algorithms converge to $\varepsilon$-Stackelberg equilibrium in $O(\nicefrac{1}{\varepsilon^2})$ and $O(\nicefrac{1}{\varepsilon^3})$ iterations, respectively, and the third, in $O(\nicefrac{1}{\varepsilon^2})$, when a Lagrangian solution oracle exists.
%\deni{We have Max oracle and LGDA/LMDA in $O(\nicefrac{1}{\varepsilon^2})$ and nested in $O(\nicefrac{1}{\varepsilon^3})$.}
As max-oracle gradient~\cite{goktas2021minmax,jin2020local} and nested GDA~\cite{goktas2021minmax} are special cases of max-oracle MD and nested MDA, respectively, our convergence bounds complement \citeauthor{goktas2021minmax}'s best iterate convergence results, now proving average iterate convergence for both algorithms.
Furthermore, our result on LMDA's convergence rate suggests the computational superiority of LMDA over nested GDA, when a Lagrangian solution oracle exists.
We also note that even when such an oracle does not exist, the Lagrangian solution can be treated as a hyperparameter of the algorithm allowing for a significant speed up in computation.

Finally, we analyze the robustness of OMD dynamics %\sadie{are we still using OMD dynamics? But both theorems in this section focus on projected OGD dynamics?}\deni{I think in terms of the story OMD is fine, we run our experiments only on OGD but that allows us to investigate OMD dynamics. Ideally, you are right, we should have had experiments with online entropic gradient descent too so that our analysis was more varied.}
by investigating online min-max Stackelberg games{, i.e., min-max Stackelberg games with arbitrary objective and constraint functions from one time step to the next}.
We prove that OMD dynamics are robust, in that even when the game changes, OMD dynamics track the changing equilibria closely, in a large class of online min-max games with independent strategy sets.
In the dependent strategy set case, we demonstrate the robustness of OMD dynamics experimentally by simulating online Fisher markets, a canonical example of an (online) min-max Stackelberg game (with dependent strategy sets) \cite{goktas2021minmax}.
%\deni{Reviewers suggested to add more on Fisher markets to the beggining but I feel like it won't be possible with space, what do you think? Alternatively, We could move the description of the Fisher market to the intro as a concrete example, and then refer to the intro in the experiments section?} 
Even when the Fisher market changes every time step, our OMD dynamics track the changing equilibria closely.
These results are somewhat surprising, because optimization problems can be highly sensitive to perturbations of their inputs \cite{ben2000robust}.
%, which extends the robustness results to dependent strategy set case.

Our findings can be summarized as follows:
\begin{itemize}[topsep=0pt]
    
    \item In repeated min-max Stackelberg games, when the outer player is a no-regret learner and the inner-player best-responds, the average of the outer player's strategies converges to their Stackelberg equilibrium strategy.
    
    \item We introduce a new type of regret we call Lagrangian regret and show that in repeated min-max Stackelberg games when both players minimize Lagrangian regret, the average of the players' strategies converge to a Stackelberg equilibrium.
    
    \item We provide convergence guarantees for max-oracle MD and nested MDA to an $\varepsilon$-Stackelberg equilibrium in $O(\nicefrac{1}{\varepsilon^2})$ and $O(\nicefrac{1}{\varepsilon^3})$ in average iterates, respectively.
    
    \item We introduce a simultaneous GDA-like algorithm, which we call LMDA, and prove that its average iterates converge to an $\varepsilon$-Stackelberg equilibrium in $O(\nicefrac{1}{\varepsilon^2})$ iterations.
    
    \item We prove that max-oracle MD and LMDA are robust to perturbations in a large class of online min-max games (with independent strategy sets).
    
    \item We run experiments with Fisher markets which suggest that max-oracle MD and LMDA are robust to perturbations in 
    %\sdeni{these}{} \amy{these is there b/c our experiments are only about Fisher markets, so i would not delete it. we cannot draw more general conclusions.} 
    these online min-max Stackelberg games.
    %(with dependent strategy sets).
\end{itemize}


% In this paper, we will define a class of no-regret learning algorithms that satisfy these desiderata in two possible game settings. First, we introduce the concept of \sdeni{pessimistic}{asymmetric} regret and show that in static convex-concave min-max Stackelberg games when the outer player uses a \sdeni{pessimistic}{asymmetric} no-regret algorithm and the inner player best responds, the dynamics converge to a Stackelberg equilibrium. This class of algorithms corresponds to a setting in which the outer player is boundedly rational and the inner player is unboundedly rational. We then prove a similar result for a setting where both players are boundedly rational and use a Lagrangian-no-regret algorithm that we introduce. We discuss the relevance of both learning settings with respect to the literature and real-world applications, and finally we apply our theoretical results to \sdeni{dynamic}{online} Fisher markets allowing us to bring results that were first proven for dynamics in Fisher markets by \citeauthor{cheung2019tracing} \cite{cheung2019tracing} to the more standard and well-understood framework of regret minimization.

\input{related}

\if 0
This paper is organized as follows.
In the next section, we present the requisite mathematical preliminaries.
In Section~\ref{sec:no-regret}, we present no-regret learning dynamics that converge in a large class of min-max Stackelberg games.
In \Cref{sec:omd}, we study the convergence and robustness properties of a particular no-regret learning algorithm, namely online mirror descent, in min-max Stackelberg games.
\fi


==> Robust No-Regret Learning in Min Max Stackelberg Games (AAMAS 2022)/omd.tex <==
\section{Online Mirror Descent}
\label{sec:omd}

%A well-known no-regret algorithm is the OMD algorithm \cite{zinkevich2003online}.
In this section, we apply the results we have derived for general no-regret learning dynamics to Online Mirror Descent (OMD) specifically \cite{nemirovskij1983problem, shalev2011online}.
%\deni{added nemirovski and yudin who invented mirror descent. OMD seems to be a folklore method, could not find any seminal paper}
We then study the robustness properties of OMD in min-max Stackelberg games.


\subsection{Convergence Analysis}

When the outer player is an OMD learner minimizing its asymmetric regret and the inner player best responds, we obtain the max-oracle mirror descent (MD) algorithm (\Cref{alg:momd}), a special case of which was first proposed by \citeauthor{jin2020local} \cite{jin2020local} for min-max games (with independent strategy sets) under the name of max-oracle GD.
\citeauthor{goktas2021minmax} \cite{goktas2021minmax} extended their algorithm from min-max games (with independent strategy sets) to min-max Stackelberg games and proved its convergence in best iterates. 
Max-oracle MD (\Cref{alg:momd}) is a further generalization of both algorithms.
%\footnote{The versions of the mirror descent algorithms in this section specialized to the case where the regularizer is the Euclidean norm
%%$\regul(\outer) = \left\| \outer\right\|_2^2$
%can be found in \Cref{sec-app:algos}.}

\begin{algorithm}[htbp]
\caption{Max-Oracle Mirror Descent (MD)}
\label{alg:momd}
\textbf{Inputs:} $\outerset, \innerset, \obj, \constr, \learnrate, \outeriters, \outer^{(0)}, \regul$ \qquad \qquad
\textbf{Output:} $\outer^{*}, \inner^{*}$
\begin{algorithmic}[1]
\For{$\outeriter = 1, \hdots, \outeriters$}
    \State Find $\inner^*(\outer[][\iter -1]) \in \br[\innerset](\outer[][\iter -1])$ 
    \State Set $\inner^{(\outeriter-1)} = \inner^*(\outer[][\iter -1])$ 
    \State Set $\langmult^{(\outeriter-1)} = \langmult^*(\outer^{(\outeriter-1)}, \inner^{(\outeriter-1)})$
    \State {\scriptsize Set $\outer[][\iter] = \argmin_{\outer \in \outerset}   \left< \grad[\outer] \lang[\outer^{(\iter-1)}]\left( \inner^{(\outeriter-1)}, \langmult^{(\outeriter-1)}\right) , \outer \right> + \frac{1}{2\learnrate[\iter]} \bregman[\regul](\outer || \outer^{(\iter-1)})$}
\EndFor
\State Set $\avgouter[][\numiters] = \frac{1}{\numiters} \sum_{\iter = 1}^\numiters \outer[][\iter]$
\State Set $\inner^*(\avgouter[][\numiters]) \in \br[\innerset](\avgouter[][\numiters])$
\State \Return $(\avgouter[][\numiters], \inner^*(\avgouter[][\numiters]))$
\end{algorithmic}
\end{algorithm}

%\deni{We are the ones who proved it for min-max Stackelberg games} 

The following corollary of \Cref{thm:pes-regret-bound}, which concerns convergence of the more general max-oracle MD algorithm in average iterates, complements \citeauthor{goktas2021minmax}'s result on the convergence of max-oracle GD (\Cref{alg:mogd}, \Cref{sec-app:algos}) in best iterates:
% \amy{check this! max-oracle or nested?}\deni{Max-Oracle!}
if the outer player employs a strategy that achieves $\varepsilon$-asymmetric regret, then the max-oracle MD algorithm is guaranteed to converge to the outer player's $(\varepsilon, 0)$-Stackelberg equilibrium strategy in average iterates after $O(\nicefrac{1}{\varepsilon^2})$ iterations, assuming the inner player best responds.

We note that 
%under \Cref{main-assum}, 
since $\val[\outerset]$ is convex, by \Cref{thm:convex-value-func}, $\val[\outerset]$ is subdifferentiable.
Moreover, for all $\widehat{\outer} \in \outerset$, $\widehat{\inner} \in \br[\innerset](\widehat{\outer})$, $\grad[\outer] \obj(\widehat{\outer}, \widehat{\inner}) + \sum_{\numconstr = 1}^\numconstrs \langmult[\numconstr]^* \constr[\numconstr](\widehat{\outer}, \widehat{\inner})$ is an arbitrary subgradient of the value function at $\widehat{\outer}$ by \citeauthor{goktas2021minmax}'s  subdifferential envelope theorem \cite{goktas2021minmax}.
We add that similar to \citeauthor{goktas2021minmax}, we assume that the optimal KKT multipliers $\langmult^*(\outer^{(\outeriter)}, \widehat{\inner}(\outer^{(\outeriter)}))$ associated with a solution $\widehat{\inner}(\outer^{(\outeriter)}))$ can be computed in constant time.

\begin{corollary}
\label{corr:max-oracle-gradient-descent}
%Suppose that \Cref{main-assum} holds.
Let $c = \max_{\outer \in \outerset} \left\| \outer \right\|$ and let $\lipschitz[\obj] =  \max_{(\widehat{\outer}, \widehat{\inner}) \in \outerset \times \innerset} \\ \left\| \grad[\outer] \obj (\widehat{\outer}, \widehat{\inner}) \right\|$.
If \Cref{alg:momd} is run on a repeated min-max Stackelberg game $(\outerset, \innerset, \obj, \constr)$, with $\learnrate[\iter] = \frac{c}{\lipschitz[\obj] \sqrt{2T}}$, for all iteration $\iter \in \iters$ and any $\outer[][0] \in \outerset$, then $(\avgouter[][\numiters], \inner^*(\avgouter[][\numiters]))$ is a $(\nicefrac{c \lipschitz[\obj] \sqrt{2}}{\sqrt{\numiters}}, 0)$-Stackelberg equilibrium.
%, i.e., $ \max_{\inner \in \innerset: \constr(\avgouter[][\numiters], \inner)} \obj(\avgouter[][\numiters], \inner) \leq \obj(\avgouter[][\numiters], \inner^*(\avgouter[][\numiters]))  \leq \min_{\outer \in \outerset} \max_{\inner \in \innerset : \constr(\outer, \inner) \geq \zeros} \obj(\outer, \inner) + \nicefrac{c \lipschitz[\obj] \sqrt{2} }{\sqrt{\numiters}}$
Furthermore, for any $\varepsilon \in (0,1)$, there exists $N(\varepsilon) \in O(\nicefrac{1}{\varepsilon^{2}})$ s.t.{} for all $\numiters \geq N(\varepsilon)$, there exists an iteration $\numiters^{*} \leq \outeriters$ s.t.\ $(\avgouter[][\numiters], \inner^*(\avgouter[][\numiters]))$ is an $(\varepsilon, 0)$-Stackelberg equilibrium.
\end{corollary}

Note that we can relax \Cref{thm:pes-regret-bound} to instead work with an approximate best response of the inner player, i.e., given the strategy of the outer player $\widehat{\outer}$, instead of playing an exact best-response, the inner player could compute a $\widehat{\inner}$ s.t.\ $\obj(\widehat{\outer}, \widehat{\inner}) \geq \max_{\inner \in \innerset : \constr(\widehat{\outer}, \inner) \geq \zeros } \obj(\widehat{\outer}) - \varepsilon$.
Moreover, the inner player could run gradient (or mirror) ascent on $\obj(\widehat{\outer}, \inner)$ to find $\widehat{\inner}$, instead of assuming a best-response oracle in \Cref{alg:momd}.
We can combine the fact that gradient ascent on Lipschitz smooth functions converges in $O(\nicefrac{1}{\varepsilon})$ iterations \cite{nemirovskij1983problem} with our novel convergence rate for max-oracle MD to conclude that the average iterates computed by nested GDA \cite{goktas2021minmax} 
% \amy{is this specific to our algo? or is it also true of Jin's? can we just say nested GDA, without referencing ourselves here?}\deni{It is specific to our algo. How about we remove the name but just cite ourselves at the end of nested GDA phrase?}\amy{ok!}
converge to an $(\varepsilon, \varepsilon)$-Stackelberg equilibrium in $O(\nicefrac{1}{\varepsilon^{3}})$ iterations.
%under \Cref{main-assum}.
If additionally, $\obj$ is strongly convex in $\inner$, then the iteration complexity can be reduced to $O(\nicefrac{1}{\varepsilon^{2}}\log(\nicefrac{1}{\varepsilon}))$. 

Similarly, we can also consider the {symmetric} case, in which both the outer and inner players minimize their Lagrangian regrets, as OMD learners with access to a Lagrangian solution oracle that returns $\langmult^* \in \argmin_{\langmult \geq 0} \min_{\outer \in \outerset} \max_{\inner \in \innerset} \lang[\outer](\inner, \langmult)$.
In this case, we obtain the \mydef{Lagrangian mirror descent ascent (LMDA)} algorithm (Algorithm~\ref{alg:lmda}).
The following corollary of \Cref{thm:lang-regret-bound} states that LMDA
%(\Cref{alg:lgda}) 
converges in average iterates to an $\varepsilon$-Stackelberg equilibrium in $O(\nicefrac{1}{\varepsilon^{2}})$ iterations.

\begin{algorithm}[htbp]
\caption{Lagrangian Mirror Descent Ascent (LMDA)}
\label{alg:lmda}
\textbf{Inputs:} $\langmult^*, \outerset, \innerset, \obj, \constr,  \learnrate[][\outer], \learnrate[][\inner], \numiters,  \outer^{(0)},  \inner^{(0)}, \regul$ \qquad
\textbf{Output:} $\outer^{*}, \inner^{*}$
\begin{algorithmic}[1]
\For{$\iter = 1, \hdots, \numiters -1$}    
    
    % \State Set $\u^{(t)} =  \u^{(t-1)} - \learnrate[\outeriter][\outer] \grad[\outer] \lang[{\outer^{(\outeriter-1)}}]\left( \inner^{(\outeriter-1)}, \langmult^{*}\right) $
    
    \State {\scriptsize Set $\outer[][\iter] = \argmin_{\outer \in \outerset}   \left< \grad[\outer] \lang[\outer^{(\iter-1)}]\left( \inner^{(\outeriter-1)}, \langmult^*\right) , \outer \right> + \frac{1}{2\learnrate[\iter]} \bregman[\regul](\outer || \outer^{(\iter)})$}

    % \State Set $\v^{(t)} =  \v^{(t-1)} + \learnrate[\outeriter][\inner] \grad[\inner] \lang[{\outer^{(\outeriter-1)}}]\left( \inner^{(\outeriter-1)}, \langmult^{*}\right) $
    
    \State {\scriptsize Set $\inner[][\iter] = \argmax_{\inner \in \innerset}   \left< \grad[\inner] \lang[\outer^{(\iter-1)}]\left( \inner^{(\iter-1)}, \langmult^*\right) , \inner \right> - \frac{1}{2\learnrate[\iter]} \bregman[\regul](\inner || \inner^{(\iter-1)})$}
    
    % \State Set $\inner^{(\iter)} = \argmin_{\inner \in \innerset} \left\{ \regul(\inner) - \left< \v^{(t)} , \inner \right> \right\}$
    
    % \State Set $\inner^{(\iter +1)} = \project[{
    % \innerset
    % }] \left( \inner^{(\iter)} + \learnrate[\iter][\inner] \grad[\inner] \lang[{\outer[][\iter]}](\inner[][\iter], \langmult^*)
    % \left[ \grad[\inner] \obj (\outer^{(\iter)}, \inner^{(\iter)}) + \sum_{\numconstr = 1}^\numconstrs \langmult[\numconstr]^* \grad[\inner]  \constr[\numconstr](\outer^{(\iter)}, \inner^{(\iter)}) \right] 
    % \right)$ 
\EndFor
\State \Return $\{(\outer[][\iter], \inner[][\iter])\}_{\iter= 1}^\numiters$
\end{algorithmic}
\end{algorithm}

\begin{corollary}
\label{cor:simu-omd}
%Suppose that \Cref{main-assum} holds.
Let $b = \max_{\outer \in \outerset} \left\| \outer \right\|$, $c = \max_{\inner \in \innerset} \left\| \inner \right\|$, and $\lipschitz[\lang] = \max_{(\widehat{\outer}, \widehat{\inner}) \in \outerset \times \innerset} \left\| \grad[\outer] \lang[{\widehat{\outer}}](\widehat{\inner}, \langmult^*) \right\|$.
 If \Cref{alg:lmda} is run on a repeated min-max Stackelberg game $(\outerset, \innerset, \obj, \constr)$, with $\learnrate[\iter][\outer] = \frac{b }{\lipschitz[\lang] \sqrt{2T}}$ and $\learnrate[\iter][\inner] = \frac{c }{\lipschitz[\lang] \sqrt{2T}}$, for all iterations $\iter \in \iters$ and any $\outer[][0] \in \outerset$, 
 %and returns $\{(\outer[][\iter], \inner[][\iter])\}_{\iter= 1}^\numiters$. Let $\avgouter[][\numiters] = \frac{1}{\numiters} \sum_{\iter = 1}^\numiters \outer[][\iter]$, $\avginner[][\numiters] = \frac{1}{\numiters} \sum_{\iter = 1}^\numiters \inner[][\iter]$, 
 then the following convergence bound holds on the saddle point residual of $(\avgouter[][\numiters], \avginner[][\numiters])$ w.r.t.\ the Lagrangian:
%\begin{align}
    $0 \leq \max_{\inner \in \innerset}  \lang[{\avgouter[][\numiters]}](\inner, \langmult^*) - \min_{\outer \in \outerset}  \lang[\outer] (\avginner[][\numiters],\langmult^*) \leq \frac{ 2\sqrt{2} \lipschitz[\lang]  }{\sqrt{\numiters}} \max\left\{ b, c\right\}$.
%\enspace .
%\end{align}
%  is a $(\nicefrac{b \lipschitz[\lang] \sqrt{2} }{\sqrt{\numiters}}, \nicefrac{c \lipschitz[\lang] \sqrt{2} }{\sqrt{\numiters}})$-Stackelberg equilibrium. 
% Furthermore, for $\varepsilon \in (0,1)$, if we choose $\numiters \geq N_\outeriters(\varepsilon) \in O(\varepsilon^{-2})$, then there exists an iteration $\numiters^{*} \leq \outeriters$ s.t.\ $(\avgouter[][\numiters], \avginner[][\numiters])$ is an $(\varepsilon, 0)$-Stackelberg equilibrium.
\end{corollary}

We remark that in certain rare cases the Lagrangian can become degenerate in $\inner$, in that the $\inner$ terms in the Lagrangian might cancel out when $\langmult^*$ is plugged back into Lagrangian, leading LMDA to not update the $\inner$ variables, as demonstrated by the following example:

\begin{example}
Consider the following min-max Stackelberg game:
$\min_{\outer[ ] \in [-1, 1]} \max_{\inner[ ] \in [-1, 1] : 0 \leq 1 - (\outer[ ] + \inner[ ])} \outer[ ]^2 + \inner[ ] + 1 $.
When we plug the optimal KKT multiplier $\langmult[ ]^* = 1$ into the Lagrangian associated with the outer player's value function, we obtain $\lang[{\outer[ ]}]( \inner[ ], \langmult[ ]) = \outer[ ]^2 + \inner[ ] +  1 - (\outer[ ] + \inner[ ]) = \outer[ ]^2 - \outer[ ] +  1$, with
$\frac{\partial \lang}{\partial \outer[ ]} = 2x - 1$ and $\frac{\partial \lang}{\partial \inner[ ]} = 0$.
It follows that the $\outer$ iterate converges to $\nicefrac{1}{2}$, but the $\inner$ iterate will never be updated, and hence unless $\inner$ is initialized at its Stackelberg equilibrium value, LMDA will not converge to a Stackelberg equilibrium.
\end{example}

In general, this degeneracy issue occurs when $\forall \outer \in \outerset, \grad[\inner] \obj(\outer, \inner) = - \sum_{\numconstr = 1}^\numconstrs \langmult[\numconstr]^* \grad[\inner] \constr[\numconstr](\outer, \inner)$.
We can sidestep the issue by restricting our attention to min-max Stackelberg games with convex-\emph{strictly}-concave objective functions, which is \emph{sufficient} to ensure that the Lagrangian is not degenerate in $\inner$ \cite{boyd2004convex}.
However, we observe in our experiments 
%(\Cref{sec:experiments})
that even for convex-non-strictly-concave min-max Stackelberg games, LMDA, specifically with regularizer $\regul(\outer) = \left\| \outer\right\|_2^2$ (i.e., LGDA; \Cref{alg:lgda}, \Cref{sec-app:algos}), converges to Stackelberg equilibrium.


\subsection{Robustness Analysis}
\label{sec:robustness}

Our analysis thus far of min-max Stackelberg games has assumed the same game is played repeatedly.
In this section, we expand our consideration to %\emph{perturbed\/} 
online min-max Stackelberg games more generally, allowing the objective function to change from one time step to the next, as in the OCO framework.
Providing dynamics that are robust to ongoing game changes is crucial, as the real world is rarely static.
%is indeed dynamic.

%Although the OMD dynamics we analyzed in the previous section describe a dynamic behavior in nature, they assume that the game and its properties, i.e., the objective function and constraints, are static and thus do not change over time.  In many real-world games, however, the game itself is subject to perturbations, in that the agents' objectives and constraints might be perturbed by external influences.  Analyzing and providing dynamics that are robust to ongoing changes in games is critical, since the real world is rarely static.

Online games bring with them a host of interesting issues.
Notably, even though the environment might change from one time step to the next, the game still exhibits a Stackelberg equilibrium during each stage of the game.
However, one cannot reasonably expect the players to play an equilibrium during each stage, since even in a repeated game setting, known game dynamics require multiple iterations before players can reach an approximate equilibrium.
Players cannot immediately best respond, but they can behave like boundedly rational agents who take a step in the direction of their optimal strategy during each iteration.
In general online games, equilibria also become dynamic objects, which can never be reached unless the game stops changing.

% As a dynamic equilibrium cannot be computed but can only be traced, this requires us to set a different set of desiderata for game dynamics in dynamic settings to quantify how closely we are tracking this dynamic equilibrium. First, it is crucial that any game dynamics in the dynamic setting should converge to a Stackelberg equilibrium if the game stops changing, as otherwise, this would imply that our game dynamics are not tracing the Stackelberg equilibrium of the game (which is changing slowly over time). Second, it is essential for the distance between the optimal strategies that could be picked by the players and the strategies determined by the game dynamics to be bounded, for some appropriate definition of distance. To date, one of the most fundamental class of learning algorithms to have been proven to converge to Nash equilibria in min-max games (with independent strategy sets) has been no-regret algorithms \cite{cesa2006noregret}. Yet, very little is known on how no-regret algorithms behave in dynamic min-max games, let alone in dynamic min-max Stackelberg games.

Corollaries~\ref{corr:max-oracle-gradient-descent} and ~\ref{cor:simu-omd} tell us that OMD dynamics are effective equilibrium-finding strategies in repeated min-max Stackelberg games.
However, they do not provide any intuition about the robustness of OMD dynamics to perturbations in the game.
In this section, we ask whether OMD dynamics can track Stackelberg equilibria when the game changes.
%Robustness is a desirable property as many real-world applications involve changing environments.
%
%In this section, we provide theoretical guarantees that show that even when the game changes at each iteration, OMD dynamics closely track the changing equilibria of the \sdeni{}{online} game.
Ultimately, our theoretical results only concern online min-max games (with independent strategy sets), for which Nash, not Stackelberg, equilibrium is the relevant solution concept.
Nonetheless, we provide experimental evidence that suggests that the results we prove may also apply more broadly to online min-max Stackelberg games (with dependent strategy sets).
We note that our our robustness analysis focuses on projected OGD dynamics, a special case of OMD dynamics, for ease of analysis.

We first consider the asymmetric setting, in which the outer player is a no-regret learner and the inner player best-responds.
In this setting, we show that when the outer player plays according to projected OGD dynamics in an arbitrary online min-max game, the outer player's strategies closely track their Nash equilibrium strategies.
The following result states that regardless of the initial strategy of the outer player, projected OGD dynamics are always within a $\nicefrac{2d}{\delta}$ radius of the outer player's Nash equilibrium strategy.

\begin{theorem}
\label{thm:robustness_gd}
Consider an online min-max game $\left\{(\outerset, \innerset, \obj[\iter]) \right\}_{\iter = 1}^\numiters$.
Suppose that, for all $\iter \in \iters$, $\obj[\iter]$ is $\mu$-strongly convex in $\outer$ and strictly concave in $\inner$, and $ \obj[\iter]$ is $\lipschitz[{\grad\obj}]$-Lipschitz smooth.
Suppose the outer player generates a sequence of actions $\{\outer[][\iter]\}_{\iter =1}^\numiters$ by using projected OGD on the loss functions $\{ \val[][\iter]\}_{\iter = 1}^\numiters$ with learning rate $\learnrate[ ] \leq \frac{2}{\mu + \lipschitz[{\grad\obj}]}$, and further suppose the inner player generates a sequence of best-responses $\{\inner[][\iter]\}_{\iter =1}^\numiters$ to each iterate of the outer player.
For all $\iter \in \iters$, let ${\outer[][\iter]}^* \in \argmin_{\outer \in \outerset} \val[][\iter](\outer) $, $\Delta^{(\iter)} = \left\|{\outer[][\iter +1]}^* -{\outer[][\iter]}^* \right\|$, and $\delta = \frac{2 \learnrate[ ] \mu  \lipschitz[{\grad\obj}] }{\lipschitz[{\grad\obj}] + \mu}$.
We then have:
%\begin{align*}
$\left\|{\outer[][\numiters]}^* - \outer[][\numiters]\right\|    \leq (1 - \delta)^{\nicefrac{\numiters}{2}} \left\|{\outer[][0]}^* - \outer[][0]\right\| + \sum_{\iter = 1}^\numiters \left( 1 - \delta \right)^{\frac{\numiters - \iter}{2}} \Delta^{(\iter)}$.
%\enspace .
%\end{align*}
%
%\noindent
If additionally, for all $\iter \in \iters$, $\Delta^{(\iter)} \leq d$, then:
%\begin{align*}
$\left\|{\outer[][\numiters]}^* - \outer[][\numiters]\right\|    \leq (1 - \delta)^{\nicefrac{\numiters}{2}} \left\|{\outer[][0]}^* - \outer[][0]\right\| + \frac{2d}{\delta}$.
%\enspace .
%\end{align*}
\end{theorem}

We can derive a similar robustness result in the symmetric setting, where the outer and inner players are both projected OGD learners.
The following result states that regardless of the initial strategies of the two players, projected OGD dynamics follow the Nash equilibrium of the game, always staying within a $\nicefrac{4d}{\delta}$ radius.

\begin{theorem}
\label{thm:robustness_lgda}
Consider an online min-max game $
% \{ \game_\iter\}_{\iter = 0}^\numiters =
\left\{(\outerset, \innerset, \obj[\iter]) \right\}_{\iter = 1}^\numiters$.
Suppose that, for all $\iter \in \iters$, $\obj[\iter]$ is $\mu_\outer$-strongly convex in $\outer$ and $\mu_\inner$-strongly concave in $\inner$, and $\obj[\iter]$ is $\lipschitz[{ \grad \obj}]$-Lipschitz smooth.
Let $\{(\outer[][\iter], \inner[][\iter])\}_{\iter =1}^\numiters$ be the strategies played by the outer and inner players, assuming that the outer player uses a projected OGD algorithm on the losses $\{ \obj[\iter](\cdot, \inner[][\iter])\}_{\iter =1}^\numiters$ with $\learnrate[\outer] = \frac{2}{\mu_\outer + \lipschitz[{\grad \obj}]}$ and the inner player uses a projected OGD algorithm on the losses $\{ - \obj[\iter](\outer[][\iter], \cdot)\}_{\iter =1}^\numiters$ with $\learnrate[\inner] = \frac{2}{\mu_\inner + \lipschitz[{\grad \obj}]}$.
For all $\iter \in \iters$, let ${\outer[][\iter]}^* \in \argmin_{\outer \in \outerset} \obj[\iter](\outer, \inner[][\iter]) $, ${\inner[][\iter]}^* \in \argmin_{\inner \in \innerset} \obj[\iter](\outer[][\iter], \inner)$, $\Delta^{(\iter)}_{\outer} = \left\|{\outer[][\iter +1]}^* -{\outer[][\iter]}^* \right\|$, $\Delta^{(\iter)}_{\inner} = \left\|{\inner[][\iter +1]}^* -{\inner[][\iter]}^* \right\|$, $\delta_\outer = \frac{2 \learnrate[ ] \mu_\outer \lipschitz[{\grad\obj}] }{\lipschitz[{\grad[\outer] \obj}] + \mu_\outer}$, and $\delta_\inner = \frac{2 \learnrate[ ] \mu_\inner \lipschitz[{\grad\obj}] }{\lipschitz[{\grad\obj}] + \mu_\inner}$.
We then have:
%
%\begin{align*}
$\left\|{\outer[][\numiters]}^* - \outer[][\numiters]\right\| + \left\|{\inner[][\numiters]}^* - \inner[][\numiters]\right\| 
%\notag \\ 
\leq (1 - \delta_\outer)^{\nicefrac{\numiters}{2}} \left\|{\outer[][0]}^* - \outer[][0]\right\| + (1 - \delta_\inner)^{\nicefrac{\numiters}{2}} \left\|{\inner[][0]}^* - \inner[][0]\right\| 
%\notag \\
+ \sum_{\iter = 1}^\numiters \left( 1 - \delta_\outer \right)^{\frac{\numiters - \iter}{2}} \Delta_\outer^{(\iter)} + \sum_{\iter = 1}^\numiters \left( 1 - \delta_\inner \right)^{\frac{\numiters - \iter}{2}} \Delta_\inner^{(\iter)}$.
%\enspace .
%\end{align*}
%
%\noindent
If additionally, for all $\iter \in \iters$, $\Delta_\outer^{(\iter)} \leq d$ and $\Delta_\inner^{(\iter)} \leq d$, and $\delta = \min\{\delta_\inner, \delta_\outer\}$, then:
%
%\begin{align*}
$\left\|{\outer[][\numiters]}^* - \outer[][\numiters]\right\|  + \left\|{\inner[][\numiters]}^* - \inner[][\numiters]\right\|
%\notag \\ 
\leq 2(1 - \delta)^{\nicefrac{\numiters}{2}} \\
\left(  \left\|{\outer[][0]}^* - \outer[][0]\right\| + \left\|{\inner[][0]}^* - \inner[][0]\right\| \right) + \frac{4d}{\delta}$.
%\enspace .
%\end{align*}
\end{theorem}

The proofs of the above theorems are relegated to \Cref{sec_app:proofs}.
These theorems establish the robustness of projected OGD dynamics for min-max games in both the asymmetric and symmetric settings by showing that the dynamics closely track the Nash equilibria in a large class of min-max games (with independent strategy sets). These results also suggest that general OMD dynamics, e.g., OMD with entropy as a regularizer, are robust to perturbation.
As we are not able to extend these theoretical robustness guarantees to min-max Stackelberg games (with dependent strategy sets), we instead ran a series of experiments with online Fisher markets, which are canonical examples of min-max Stackelberg games \cite{goktas2021minmax}, to investigate the empirical robustness guarantees of projected OGD dynamics for this class of min-max Stackelberg games.


==> Robust No-Regret Learning in Min Max Stackelberg Games (AAMAS 2022)/prelim.tex <==
\section{Mathematical Preliminaries}
\label{sec:prelim}


\paragraph{Notation}

We use Roman uppercase letters to denote sets (e.g., $X$),
% calligraphic uppercase letters to denote correspondences (e.g., $\calX$),\amy{do we still have any correspondences? we might not need this.}
bold uppercase letters to denote matrices (e.g., $\allocation$), bold lowercase letters to denote vectors (e.g., $\price$), and Roman lowercase letters to denote scalar quantities, (e.g., $c$).
We denote the $i$th row vector of a matrix (e.g., $\allocation$) by the corresponding bold lowercase letter with subscript $i$ (e.g., $\allocation[\buyer])$.
Similarly, we denote the $j$th entry of a vector (e.g., $\price$ or $\allocation[\buyer]$) by the corresponding Roman lowercase letter with subscript $j$ (e.g., $\price[\good]$ or $\allocation[\buyer][\good]$).
We denote the vector of ones of size $\numbuyers$ by $\ones[\numbuyers]$.
We denote the set of integers $\left\{1, \hdots, n\right\}$ by $[n]$, the set of natural numbers by $\N$, the set of positive natural numbers by $\N_+$ the set of real numbers by $\R$, the set of non-negative real numbers by $\R_+$, and the set of strictly positive real numbers by $\R_{++}$.
We denote the orthogonal projection operator onto a convex set $C$ by $\project[C]$, i.e., $\project[C](\x) = \argmin_{\y \in C} \left\|\x - \y \right\|^2$. 
Given a sequence of iterates $\{ \z^{(\iter)} \}_{\iter =1}^\numiters \subset Z$, we denote the average iterate $\bar{\z}^{(\numiters)} = \frac{1}{\numiters} \sum_{\iter =1 }^\numiters \z^{(\iter)}$.


\paragraph{Game Definitions}

A \mydef{min-max Stackelberg game}, $(\outerset, \innerset, \obj, \constr)$, is a two-player, zero-sum game, where one player, who we call the \mydef{outer}
%, or $\outer$-, 
player (resp.\ the \mydef{inner}
%, or $\inner$-, 
player), is trying to minimize their loss (resp.\ maximize their gain), defined by a continuous \mydef{objective function} $\obj: X \times Y \rightarrow \mathbb{R}$, by choosing a strategy from their non-empty and compact \mydef{strategy set} $\outerset \subset \R^\outerdim$, and (resp. $\innerset \subset \R^\innerdim$) s.t.\ $\constr(\outer, \inner) \geq 0$ where $\constr(\outer, \inner) = \left(\constr[1](\outer, \inner), \hdots, \constr[\numconstrs](\outer, \inner) \right)^T$ with $\constr[\numconstr]: \outerset \times \innerset \to \R$ continuous.
A strategy profile $(\outer, \inner) \in \outerset \times \innerset$ is said to be \mydef{feasible} iff for all $\numconstr \in [\numconstrs]$, $\constr[\numconstr](\outer, \inner) \geq 0$.
The function $\obj$ maps a pair of strategies taken by the players $(\outer, \inner) \in \outerset \times \innerset$ to a real value (i.e., a payoff), which represents the loss (resp.\ the gain) of the outer player (resp.\ the inner player).
A min-max game is said to be convex-concave if the objective function $\obj$ is convex-concave and $\outerset$ and $\innerset$ are convex sets.

%One way to see this game is as a \mydef{Stackelberg game}, i.e., a sequential game with two players, where 
% \samy{WLOG, we assume the minimizing player moves first and the maximizing player moves second.}{}
% \amy{was that necessary?}
The relevant solution concept for Stackelberg games is the \mydef{Stackelberg equilibrium (SE)}:
A strategy profile $\left( \outer^{*}, \inner^{*} \right) \in \outerset \times \innerset$ s.t.\ $\constr \left( \outer^{*}, \inner^{*} \right) \geq \zeros$ is an $(\epsilon, \delta)$-SE if
%\begin{equation}
$\max_{\inner \in \innerset : \constr \left( \outer^{*}, \inner \right) \geq 0} \obj \left( \outer^{*}, \inner \right) - \delta \leq \obj \left( \outer^{*}, \inner^{*} \right) \leq \min_{\outer \in \outerset} \max_{\inner \in \innerset : \constr(\outer, \inner) \geq 0} \obj \left( \outer, \inner \right) + \epsilon$.
%\enspace .
%\end{equation}
%\end{definition}
%
%\noindent
Intuitively, a $(\varepsilon, \delta)$-SE is a point at which the outer player's (resp.\ inner player's) payoff is no more than $\varepsilon$ (resp.\ $\delta$) away from its optimum.
A $(0,0)$-SE is guaranteed to exist in min-max Stackelberg games \cite{goktas2021minmax}.
Note that when $\constr(\outer, \inner) \geq \zeros$, for all $(\outer, \inner) \in \outerset \times \innerset$, the game reduces to a min-max game (with independent strategy sets).
% ,for which, by the minimax theorem, a Nash equilibrium is guaranteed to exist \cite{neumann1928theorie}.%
%%% SPACE
%\footnote{When Nash equilibria exist, Nash and Stackelberg equilibria coincide.}

In a min-max Stackelberg game, the outer player's \mydef{best-response set} $\br[\outerset] \subset \outerset$, defined as $\br[\outerset] = \argmin_{\outer \in \outerset} \val[\outerset](\outer)$, is independent of the inner player's strategy, while the inner player's \mydef{best-response correspondence} $\br[\innerset] : \outerset \rightrightarrows \innerset$, defined as $\br[\innerset](\outer) = \argmax_{\inner \in \innerset: \constr(\outer, \inner) \geq 0} \val[\innerset](\inner; \outer)$,
depends on the outer player's strategy.
A $(0,0)$-Stackelberg equilibrium $(\outer^*, \inner^*) \in \outerset \times \innerset$ is then a tuple of strategies such that $(\outer^*, \inner^*) \in \br[\outerset] \times \br[\innerset](\outer^*)$. 


An \mydef{online min-max Stackelberg game}, $\left\{ \left( \outerset, \innerset, \obj[\iter], \constr[][\iter] \right) \right\}$, 
%\amy{i propose we drop all the $t=1$ to $T$ notation from these sequences everywhere. it takes up alot of space, and it is not really part of the game. the game could go longer, but we stop learning after $T$ iterations.} 
is a sequence of min-max Stackelberg games played for $\numiters$ time periods.
We define the players' value functions at time $\iter$ in a online min-max Stackelberg game in terms of $\obj[\iter]$ and $\constr[][\iter]$.
\if 0
We define the \mydef{the outer player's value function} at time $\iter$ by $\val[\outerset][\iter](\outer) = \max_{\inner \in \innerset : \constr[][\iter](\outer, \inner) \geq \zeros} \obj[\iter](\outer, \inner)$, and the \mydef{inner player's value function} given the outer player's strategy $\outer$, $\val[\innerset][\iter](\inner; \outer) = \obj[\iter](\inner; \outer)$.
\fi
% When $\iters \subseteq \R_+$, we have $\{ \game_\iter\}_{\iter \in \iters}$ is called a continuous time dynamic min-max game with dependent strategy sets, and when $\iters \subseteq \in \N_+$, we have a discrete time dynamic min-max game with dependent strategy sets. 
Note that when $\constr[][\iter](\outer, \inner) \geq 0$ for all $\outer \in \outerset, \inner \in \innerset$ and all time periods $\iter \in \iters$, the game reduces to a online min-max game (with independent strategy sets).
Moreover, if for all $\iter, \iter' \in \iters, \obj[\iter] = \obj[\iter']$, and $\constr[][\iter] = \constr[][\iter']$, then the game reduces to a \mydef{repeated min-max Stackelberg game}, which we denote simply by $(\outerset, \innerset, \obj, \constr)$.
%\sadie{Do we need to change the notation to differentiate a single min-max Stackelberg game and a repeated min-max Stackelberg game?}
%\footnote{We note that we use the tuple $(\outerset, \innerset, \obj, \constr)$ to refer both to a static, and repeated min-max Stackelberg game. When not clear from context, we make sure to state what type of game the tuple refers to.}

\paragraph{Assumptions}
All the theoretical results on min-max Stackelberg games in this paper rely on the following assumption(s):
%
\sdeni{
% \begin{assumption}
% \label{main-assum}
% 1. (\emph{Slater's condition} \cite{slater1959convex, slater2014convex})~ $\forall \outer \in \outerset, \exists \widehat{\inner} \in \innerset$ s.t.\ $g_{\numconstr}(\outer, \widehat{\inner}) > \zeros$, for all $\numconstr = 1, \ldots, \numconstrs$; 2.~$\obj, \constr[1], \ldots, \constr[\numconstrs]$ are continuous and convex-concave; and 3.~$\grad[\outer] f, \grad[\outer] \constr[1], \ldots, \grad[\outer] \constr[\numconstrs]$ are well-defined for all $(\outer, \inner) \in \outerset \times \innerset$ and continuous in $(\outer, \inner)$; 4.~$\outerset$ and $\innerset$ are convex.
% %\deni{I cannot see this assumption stated anywhere oddly but it should be here!!} \amy{is this assumption missing from the NeurIPS paper as well?}\deni{Yes, it is missing but in the NeurIPS paper we state the convexity assumption in the theorem because it can be loosened sometimes, but we forget to state it for some lemmas, we have to fix that!}
% \end{assumption}
}{

\begin{assumption}
\label{main-assum}
1.~(Slater's condition)
$\forall \outer \in \outerset, \exists \widehat{\inner} \in \innerset$ s.t.\ $g_{\numconstr}(\outer, \widehat{\inner}) > 0$, for all $\numconstr \in [\numconstrs]$;
% 1.~$\obj(\outer, \inner), \mu \constr[1](\outer, \inner), \ldots, \mu \constr[\numconstrs](\outer, \inner)$ are continuous, convex in $(\mu, \outer)$ over the set $\R_+ \times \outerset$, for all $\inner \in \innerset$, and concave in $\inner$ over the set $\innerset$, for all $(\mu, \outer) \in \R_+ \times \outerset$;
% %, i.e., convex in $\outer$ and concave in $\inner$;
%\deni{If you look at the proof of \Cref{thm:convex-value-func}, you'll notice that that convex-concavity of the constraints is necessary for the value function of the outer player to be convex. If this assumption does not hold than the problem becomes NP-hard. Note this assumption is also in the same as the assumptions made by \cite{ho2018online} for RO};
2.~$\grad[\outer] f, \grad[\outer] \constr[1], \ldots, \grad[\outer] \constr[\numconstrs]$ are continuous;
%in $(\outer, \inner)$ \amy{what does it mean to be continuous in this pair?}\deni{It is just your regular definition of continuity, you could just remove "the pair part" and it would still mean the same!}
and 3.a.~$\obj$ is continuous and convex-concave, 3.b.~$\mu \constr[1](\outer, \inner), \ldots,$ $\mu \constr[\numconstrs](\outer, \inner)$ are continuous, convex in $(\mu, \outer)$ over the set $\R_+ \times \outerset$, for all $\inner \in \innerset$, and concave in $\inner$ over the set $\innerset$, for all $(\mu, \outer) \in \R_+ \times \outerset$.
% \sdeni{}{and $\outerset$, $\innerset$ are convex}.
\end{assumption}
}

We note that these assumptions are in line with previous work geared towards solving min-max Stackelberg games 
%with first-order methods
\cite{goktas2021minmax}.
Part 1 of \Cref{main-assum},
Slater's condition, is a standard constraint qualification condition \cite{boyd2004convex}, which is needed to derive the optimality conditions for the inner player's maximization problem; without it the problem becomes analytically intractable.
Part 2 of \Cref{main-assum} ensures that the value function of the outer player is continuous and convex (\cite{goktas2021minmax}, Proposition A1), so that the problem affords an efficient solution.
Part 3 of \Cref{main-assum} can be replaced by a weaker, subgradient boundedness assumption; however, for simplicity, we assume this stronger condition.
Finally, Part 4 of \Cref{main-assum} guarantees that projections are polynomial-time operations.

Under \Cref{main-assum}, the following property holds of the outer player's value function.

\begin{proposition}[\cite{goktas2021minmax}, Proposition B.1]
\label{thm:convex-value-func}
Consider a min-max Stackelberg game $(\outerset, \innerset, \obj, \constr)$ and suppose that \Cref{main-assum} holds, then the outer player's value function $\val(\outer) = \max_{\inner \in \innerset : \constr(\outer, \inner) \geq \zeros} \obj(\outer, \inner)$ is continuous and convex.
\end{proposition}


\paragraph{Additional Definitions}
%
%We define several concepts that are needed in our convergence proofs.
Given two normed spaces $(\outerset, \|\cdot \|)$ and $(\innerset, \|\cdot \|)$, the function $\obj: \outerset \to \innerset$ is
%said to be
$\lipschitz[\obj]$-\mydef{Lipschitz-continuous} iff $\forall \outer_1, \outer_2 \in X, \left\| \obj(\outer_1) - \obj(\outer_2) \right\| \leq \lipschitz[\obj] \left\| \outer_1 - \outer_2 \right\|$.
If the gradient of $\obj$, $\grad \obj$, is $\lipschitz[\grad \obj]$-Lipschitz-continuous, we refer to $\obj$ as $\lipschitz[\grad \obj]$-\mydef{Lipschitz-smooth}.
A function $\obj: A \to \R$ is $\mu$-\mydef{strongly convex} if $\obj(\outer_1) \geq \obj(\outer_2) + \left< \grad[\outer] \obj(\outer_2), \outer_1 - \outer_2 \right> + \nicefrac{\mu}{2} \left\| \outer_1 - \outer_1 \right\|^2$, and $\mu$-\mydef{strongly concave} if $-\obj$ is $\mu$-strongly convex.


\paragraph{Online Convex Optimization}

%\mydef{OCO} is a toolbox used to solve online convex optimization problems, 

An \mydef{online convex optimization problem (OCP)} is a decision problem in a dynamic environment which comprises a finite time horizon $\numiters$, a compact, convex feasible set $\outerset$, and a sequence of convex differentiable loss functions $\{\loss[][\iter] \}_{\iter = 1}^\numiters$, where $\loss[][\iter]: \outerset \to \R$ for all $\iter \in [\numiters]$.
A solution to an OCP is a sequence $\{ \outer^{(\iter)} \}_{\iter = 1}^\numiters$ with each $\outer^{(\iter)} \in \outerset$.
A preferred solution is one that minimizes \mydef{average regret}, given by
% \amy{don't you want to define this, where $\outer$ depends on the iteration: maybe
% $\regret[][\numiters](\left\{ \outer^{\iter} \right\}, \outer)$?}\deni{Feels too dangerous, High risk low reward. We have to change it everywhere and a mistake will definitely slip in.}
% \amy{disagree. let's proofread carefully! more longer notation is more room for typos!}
% \amy{also, your def'n just seem wrong. there are two free variables, but you only mention that Regret is a function of one of them, $\outer$, not $\left\{ \outer^{\iter} \right\}_{\iter=1}^{\numiters}$.}
% 
% \amy{another thing we can write, overloading notation is: $$\regret[][\numiters](\left\{ \outer^{\iter} \right\}) = \max_{\outer \in \outerset} \regret[][\numiters](\left\{ \outer^{\iter} \right\}, \outer)$$ but i think it is really important that $\left\{ \outer^{\iter} \right\}$ be one of the arguments to Regret. it doesn't seem correct to me without it!}
%
%\begin{align*}
$\regret[][\numiters](\left\{ \outer^{\iter} \right\}, \outer) = \sum_{\iter = 1}^\numiters \frac{1}{\numiters}\loss[][\iter](\outer^{(\iter)}) - \sum_{\iter = 1}^\numiters \frac{1}{\numiters} \loss[][\iter](\outer)$,
%\enspace ,
%\end{align*}
for all $\outer \in \outerset$.
%
Overloading notation, we also write $\regret[][\numiters](\left\{ \outer^{\iter} \right\}) = \max_{\outer \in \outerset} \regret[][\numiters](\left\{ \outer^{\iter} \right\}, \outer)$.
%, i.e., $\sum_{\iter = 1}^\numiters \frac{1}{\numiters}\loss[][\iter](\outer^{(\iter)}) - \min_{\outer \in \outerset} \sum_{\iter = 1}^\numiters \frac{1}{\numiters} \loss[][\iter](\outer)$.
An algorithm $\algo$ 
% \amy{i don't think the type of the algorithm is correct. but i also don't think we need it. the English is enough.} 
that takes as input a sequence of loss functions and outputs decisions such that  $\regret[][\numiters](\algo(\{\loss[][\iter] \}) \to 0$ 
% $\sum_{\iter = 1}^\numiters \frac{1}{\numiters}\loss[][\iter](\algo(\{\loss[][\iter] \}_{\iter = 1}^\numiters)) - \min_{\outer \in \outerset} \sum_{\iter = 1}^\numiters \frac{1}{\numiters} \loss[][\iter](\outer) \to 0$
% \amy{as it is written here, it looks like the algo can make decisions based on future loss functions, which it should not be able to do!}
% \amy{also, with the def'n as i proposed, you need only say $\regret[][\numiters](\algo(\{\loss[][\iter] \}) \to 0$}
as $\numiters \to \infty$ is called a \mydef{no-regret algorithm}.

For any differentiable convex function $\regul: \outerset \to \R$, the \mydef{Bregman divergence} between two vectors $\w, \u \in \outerset$ is defined as follows:
%\begin{align}
    $\bregman[\regul](\w||\u)=\regul(\w)-(\regul(\u)+\left<\grad \regul(\u), (\w-\u)\right>$.
    %\label{2.12}
%\end{align}
One first-order no-regret learning algorithm is \mydef{Online Mirror Descent (OMD)}, defined as follows for some initial iterate $\outer^{(0)} \in \outerset$, a fixed learning rate $\learnrate[ ] > 0$, and a strongly convex regularizer $\regul$:
%\begin{align*}
$\outer^{(\iter+1)} = \argmin_{\outer \in \outerset} \left< \grad[\outer] \loss[][\iter](\outer^{(\iter)}), \outer \right> + \frac{1}{2\learnrate[ ]} \bregman[\regul](\outer || \outer^{(\iter)})$.
%\enspace .
%\end{align*}
%
When $\regul(\outer) = \frac{1}{2} \left\|\outer \right\|^2_2$, OMD reduces to \mydef{projected online gradient descent (OGD)}, given by the update rule:
%\begin{align*}
    $\outer^{(\iter + 1)} = \proj[\outerset] \left(\outer^{(\iter)} - \eta \grad[\outer] \loss[ ][\iter] (\outer^{(\iter)}) \right)$. 
%\enspace .
%\end{align*}
\if 0
\deni{Delete this this next bit from here}  
One first-order method that solves OCPs is \mydef{Online Mirror Descent (OMD)}.
For some initial iterates $\u^{(0)} = 0$ and $\outer[][\iter] \in \outerset$, OMD performs the following update in the dual space $\outerset^*$ at each time step $\iter$:  $\u^{(t+1)} = \u^{(t)} - \learnrate[ ] \grad[\outer] \loss[ ][\iter](\outer^{(\iter)})$, and then projects the iterate computed in the dual space $\outerset^*$ back into the primal space $\outerset$: $\outer^{(\iter + 1)} = \argmin_{\outer \in \outerset} \left\{ \regul(\outer) - \left< \u^{(t+1)} , \outer \right> \right\}$, where $\regul : \outerset \to \R$ is a strongly-convex differentiable function.
\deni{to here}
\fi
%
%\enspace .
%\end{align}
%where $\proj[\outerset](\u) = \argmin_{\outer \in \outerset} \left\| \u - \outer \right\|_2^2$
The next theorem bounds the \mydef{average regret} of OMD \cite{kakade2012regularization}:

% \begin{theorem}
% %\amy{is this true for all norms $\left\| \right\|$?}\deni{Yes!}
% Let $c = \max_{\outer \in \outerset} \left\| \outer \right\|$, and let $\{\loss[ ][\iter] \}$ be a sequence of functions s.t.\ for all $\iter \in \N_+$, $\loss[ ][\iter]: \R^\outerdim \to \R$ is $\lipschitz$-Lipschitz w.r.t. the dual norm $\left\| \cdot \right\|_*$.
% Then, if $\learnrate[ ] = \frac{c}{\lipschitz\sqrt{2T}}$, projected OGD \amy{do we have to generalize this result to OMD, so that the later theorems go thru for the new, more general algos?} achieves average regret bounded as follows:
% %\begin{align}
%     % \sum_{\iter = 1}^\numiters \loss[][\iter](\outer^{(\iter)}) - \min_{\outer \in \outerset} \sum_{\iter = 1}^\numiters \loss[][\iter](\outer) \leq c \lipschitz \sqrt{2\numiters}\\
% % \samy{$\sum_{\iter = 1}^\numiters \frac{1}{\numiters}\loss[][\iter](\outer^{(\iter)}) - \min_{\outer \in \outerset} \sum_{\iter = 1}^\numiters \frac{1}{\numiters}\loss[][\iter](\outer) \leq c \lipschitz \sqrt{\frac{2}{\numiters}}$.}
% %\end{align}
% $\regret[][\numiters](\left\{ \outer^{\iter} \right\}) \leq c \lipschitz \sqrt{\frac{2}{\numiters}}$.
% \end{theorem}

\begin{theorem}
%\amy{is this true for all norms $\left\| \right\|$?}\deni{Yes!}
Suppose that the OMD algorithm generates a sequence of iterates $\{ \outer^{(\iter)}\}$ when run with a $1$-strongly convex regularizer $\regul$%
\footnote{This assumption is without loss of generality, since any $m$-strongly-convex regularizer can be transformed into a $1$-strongly-convex regularizer}.
Let $c = \max_{\outer \in \outerset, \iter \in \iters} \bregman[\regul](\outer || \outer^{(\iter)})$, and let $\{\loss[ ][\iter] \}$ be a sequence of functions s.t.\ for all $\iter \in \N_+$, $\loss[ ][\iter]: \R^\outerdim \to \R$ is $\lipschitz$-Lipschitz w.r.t. the dual norm $\left\| \cdot \right\|_*$.
Then, if $\learnrate[ ] = \frac{c}{\lipschitz\sqrt{2T}}$, OMD achieves average regret bounded as follows:
$\regret[][\numiters](\left\{ \outer^{\iter} \right\}) \leq c  \lipschitz \sqrt{\nicefrac{2}{\numiters}}$.
\end{theorem}

\if 0
\paragraph{Lyapunov Dynamical Systems (LDS)} A dynamical system $\lds = (\outer[][0], \evolve)$ is a tuple consisting of an initial control variable vector $\outer[][0] \in \outerset$, and an evolution rule, $\evolve: \outerset \to \outerset$ which denote the evolution function from one time step to the other $\outer[][\iter +1] = \evolve(\outer[][\iter])$, where $\outerset \subset \R^\outerdim$. A system is called a Lyapunov Dynamic System (LDS) if it admits a Lyapunov function $\lf: \outerset \to \R_+$ such that 1) for every fixed point of $\evolve$ such that $\evolve(\outer^*) = \outer^*$, we have $\lf(\outer^*) = 0$, and 2) for every $\outer \in \outerset$, we have $\lf(\evolve(\outer)) \leq \lf(\outer)$.

\fi

==> Robust No-Regret Learning in Min Max Stackelberg Games (AAMAS 2022)/related.tex <==
\paragraph{Related Work}

% \samy{Several algorithms have been proposed to solve convex-concave min-max Stackelberg games \cite{segundo2012evolutionary, shizimu1981stackelberg, shimizu1980minmax}.
% Recently, \citeauthor{goktas2021minmax} 
% \cite{goktas2021minmax} developed the first such algorithms with polynomial-time guarantees.}{}
% \amy{not needed here, since we already cited this work.}

% Further, min-max Stackelberg games are mathematically related to the abstract economies first studied by \citeauthor{arrow-debreu} \cite{arrow-debreu}; however, the solution concept that has been the focus of most work in this literature is generalized Nash equilibrium \cite{facchinei2007generalized, facchinei2010generalized}, which, like Stackelberg, is a weaker solution concept than Nash equilibrium, but which makes the arguably unreasonable assumption that the players move simultaneously and nonetheless satisfy the constraint dependencies on their strategies imposed by one another's moves.

% A related problem setting to that of min-max Stackelberg games is extensive-form games with dependent strategy sets, for which algorithms have been proposed when payoffs are bilinear \cite{davis2019solving} or have a specific convex-concave structure \cite{farina2019regret}.

Stackelberg games \cite{stackelberg1934marktform} have found important applications in the domain of security (e.g., \cite{nguyen2016ssg, sinha2018stackelberg}) and environmental protection (e.g., \cite{fang2016sgsg}).
These applications have thus far been modelled as Stackelberg games with independent strategy sets.
Yet, the increased expressiveness of Stackelberg games with dependent strategy sets may make them a better model of the real world, as they provide the leader with more power to achieve a better outcome by constraining the follower's choices.
%\amy{we have to say that there are applications where you really want to model the constraints on the follower's choices, and if you don't model them, then your losing information, and your solution is not as good as it could be.}

The study of algorithms that compute competitive equilibria in Fisher markets was initiated by \citeauthor{devanur2002market} \cite{devanur2002market}, who provided a polynomial-time method for solving these markets assuming linear utilities.
%\citeauthor{jain2005market} \cite{jain2005market} subsequently extended these polynomial-time computation guarantees to a large class of Fisher markets.
%Recently, \citeauthor{gao2020polygm} \cite{gao2020polygm} proposed first-order methods for solving Fisher markets (only; not general min-max Stackelberg games), assuming linear, quasilinear, and Leontief utilities, as such methods can be more efficient when markets are large.
More recently, \citeauthor{cheung2019tracing} \cite{cheung2019tracing} studied two price adjustment processes, t\^atonnement and proportional response dynamics, in dynamic Fisher markets and showed that these price adjustment processes track the equilibrium of Fisher markets closely even when the market is subject to change.

%We provide a detailed discussion of recent progress on solving min-max games in both the convex-concave and non-convex-concave cases in \Cref{sec-app:related}.
The computation and learning of Nash and generalized Nash equilibrium in min-max games (with independent strategy sets) has been attracting a great deal of attention recently, because of the relevance of these problems to machine learning \cite{daskalakis2020complexity, abernethy2019last, daskalakis2018last, daskalakis2018limit, diakonikolas2021efficient}, specifically generative adversarial learning \cite{goodfellow2014generative}. \amy{add references to GANs here, including Ian Goodfellow}


==> Robust No-Regret Learning in Min Max Stackelberg Games (AAMAS 2022)/robust.tex <==
\section{Robustness of Online Mirror Descent Dynamics}

In dynamic min-max Stackelberg games, if the outer player is unboundedly rational then the optimal game dynamics for the outer player will simply be to best respond, i.e., playing strategy $\outer^* \in \br[\outerset]$, in which case $\outer^*$ is the Stackelberg equilibrium strategy of the outer player. However, as previously mentioned, it is not sensible to expect players to play their Stackelberg equilibrium strategy at each time period as even in the static setting players cannot compute their Stackelberg equilibrium strategy in a single time period. Note that this observation is independent from the dynamics that the inner player might choose to follow, as the best response set of the outer player is independent of the inner player's action due to the order of play. As a result, not only the study of a setting where the leader is unboundedly rational is not interesting but it is also uninteresting. Hence, throughout this paper, we will assume that the outer player is boundedly rational, in that they cannot play a best-response in a single time period. In this section we will consider an assymetric setting in which the outer player is boundedly rational and the inner player is unboundedly rational. In such a setting, the outer player cannot best respond, but the inner player's optimal strategy $\inner$  is to simply best respond to the strategy picked by the outer player $\outer$, i.e., $\inner \in \br[\innerset](\outer)$.

==> Robust No-Regret Learning in Min Max Stackelberg Games (AAMAS 2022)/todo.tex <==
% \textbf{List of things to do:}\\
% \begin{enumerate} 
% \item add proof with approximate max-oracle
% \end{enumerate}

==> robust.tex <==
\section{Robustness of Online Mirror Descent Dynamics}

In dynamic min-max Stackelberg games, if the outer player is unboundedly rational then the optimal game dynamics for the outer player will simply be to best respond, i.e., playing strategy $\outer^* \in \br[\outerset]$, in which case $\outer^*$ is the Stackelberg equilibrium strategy of the outer player. However, as previously mentioned, it is not sensible to expect players to play their Stackelberg equilibrium strategy at each time period as even in the static setting players cannot compute their Stackelberg equilibrium strategy in a single time period. Note that this observation is independent from the dynamics that the inner player might choose to follow, as the best response set of the outer player is independent of the inner player's action due to the order of play. As a result, not only the study of a setting where the leader is unboundedly rational is not interesting but it is also uninteresting. Hence, throughout this paper, we will assume that the outer player is boundedly rational, in that they cannot play a best-response in a single time period. In this section we will consider an assymetric setting in which the outer player is boundedly rational and the inner player is unboundedly rational. In such a setting, the outer player cannot best respond, but the inner player's optimal strategy $\inner$  is to simply best respond to the strategy picked by the outer player $\outer$, i.e., $\inner \in \br[\innerset](\outer)$.

==> todo.tex <==
% \textbf{List of things to do:}\\
% \begin{enumerate} 
% \item add proof with approximate max-oracle
% \end{enumerate}
